Bounded Situation Calculus Action Theories

In this paper, we investigate bounded action theories in the situation calculus. A bounded action theory is one which entails that, in every situation, the number of object tuples in the extension of fluents is bounded by a given constant, although such extensions are in general different across the infinitely many situations. We argue that such theories are common in applications, either because facts do not persist indefinitely or because the agent eventually forgets some facts, as new ones are learnt. We discuss various classes of bounded action theories. Then we show that verification of a powerful first-order variant of the mu-calculus is decidable for such theories. Notably, this variant supports a controlled form of quantification across situations. We also show that through verification, we can actually check whether an arbitrary action theory maintains boundedness.

==> 50-verification-old.tex <==

\section{Verification  of Bounded Action Theories}
%%
We can now show that
verifying $\mu\L$ temporal properties against 
bounded action theories is decidable. 
%%
In this section we focus on action theories with complete information
on the initial situation, described as a (bounded) database.  In the
next section we generalize our results to the cases with incomplete
information on the initial situation.
%%
Our main result is the following.
\begin{theorem}\label{th:dec-verif}
  If $\D$ is a bounded action theory with initial situation described
  by a (bounded) database, and $\Phi$ a closed $\mu\L$ formula, then
  verifying whether $\D\models \Phi$ is decidable.
\end{theorem}
%%
%%We next describe the schema of the proof of this result.

The proof is structured as follows.
% %%
% Firstly, observe that since $\D_0$ is a finite set of
% facts, $\D$ admits a single model $\M$ (up to
% isomorphism), which is obviously infinite, as it 
% contains the situation tree.
% Moreover, even though the number of facts
% that are true at each situation is bounded, 
% if we consider all the situations, 
% the global number of such facts is unbounded.
% Thus, the verification task cannot be carried out by 
% direct inspection of $\M$.
% %%
%%
The first step is to get rid of action terms in formulas (cf.\ Th.~\ref{prop:sitcalc-fo-act}), and observe
that $\mu\L$ can be equivalently interpreted over a certain kind of
transition systems which do not necessarily reflect the tree structure
of the situation tree (cf.\ Th.~\ref{prop:sitcalc-fo} and Th.~\ref{th:InducedTS}).

% of the proof consists of abstracting from the situation tree. 
% This is done by observing that the projection of $\M$ on a given
% situation is a FOL interpretation, and that formulas uniform in
% the situation have an equivalent FO counterpart in such an interpretation
% (cf.\ Th.~\ref{prop:sitcalc-fo-act} and Th.~\ref{prop:sitcalc-fo}).
% This allows us to disallow action terms in $\mu\L$ 
% and to provide an alternative semantics of $\mu\L$ 
% based on transition systems, where situations are irrelevant.


%%This allows us to build a transition system A-bisimilar to the 
%%one induced by the model, 
%%but where situations are not present.
%%that does not consider situation at all.

In the second step, we introduce the notions
%%, well-studied in databases, 
of: 
{\em active domain} \cite{AbHV95}, 
i.e., the domain containing all the objects occurring in the extension 
of the predicates (fluents at a given situation),
\emph{active-domain isomorphism}, i.e.,
standard isomorphism restricted to active domains,
and \emph{active-domain bisimulation},  %i.e.,
a variant of standard bisimulation which requires 
bisimilar states to be active-domain isomorphic.
%%
Then we prove that 
active-domain bisimilar transition systems 
preserve
{\em domain-independent $\mu\L$ (closed) formulas} (cf.~Th.~\ref{mu-calc-iff}), 
i.e., formulas whose evaluation of FO components 
depends only on the active domain.
%%
%%It is well known that \emph{domain-independent} formulas
%%can be interpreted over the active domain, 
%%instead of the whole interpretation domain.
%%Moreover, we define the notion of 
%%\emph{active-domain isomorphism} between FO interpretations.
%%
%%and, using the notion of  \emph{active-domain isomorphism}, we first prove that 
%%if two transition systems are bisimilar modulo active-domain isomorphism 
%%of states, they satisfy the same
%%domain-independent $\mu\L$ formulas (cf.~Th.~\ref{mu-calc-iff}).
%%

In the third and fundamental step 
we show how to actually construct 
%%
%%focuses on domain-independent formulas.
%% 
%%Then, we exploit this result to
%%construct 
an abstract, finite-state transition system that is active-domain
bisimilar to the one induced by \emph{the} model of the action theory.
%%
We make use of the assumption that situations are bounded, and 
%%In particular, we exploit both the assumption that situations are bounded
exploit the specific structure of successor state and action precondition axioms,
to devise a bound on the number of distinct objects required
to maintain active-domain isomorphisms between 
states (cf.\ Th.~\ref{th:ind-ts-bis} and~\ref{th:abs-exec}).
%%
With this we prove the decidability result for domain-independent 
$\mu\L$ formulas (cf.\ Th.~\ref{th:abs-th}).

In the final step, we generalize the above result to generic 
$\mu\L$ formulas (cf.~Th.~\ref{th:libkin}),
by observing that any FO formula interpreted over
standard names admits an equivalent, domain-independent 
formula --see, e.g., Th.~5.6.3 in~\cite{Libkin07}.
%%a part of which is interpreted over the current active
%%domain while another part, dealing with equalities over object out of
%%the active domain becomes essentially propositional   
%%Based on this, our result extends immediately to full $\mu\L$ .
%%
The rest of the section details these steps.



\subsection{Suppressing Action and Situation Terms}
We first prove that, under the assumption
that action types are finite and actions are domain closed, 
we can remove action terms from
uniform situation calculus formulas, 
including situation suppressed formulas, 
without loss of generality.

% the evaluation of precondition and successor state axioms
% can be reduced to the evaluation of formulas where no 
% action types nor situations occur. 
% %%
% Specifically, Th.~\ref{prop:sitcalc-fo-act} 
% shows how, for fixed action types, a formula 
% $\varphi$ can be rewritten as an action-term 
% free formula $\varphi'$ equivalent to $\varphi$,

% For an action theory $\D$, consider a model $\M$ over an object domain $\Delta\subseteq\N$, 
% and let $\vec x$ range over objects,
% $\vec a$ over actions, and $s$ over situation terms.
%%For a situation-calculus formula $\varphi$, $\const(\varphi)$
%%denotes the constants from $C$ occurring in $\varphi$.


\begin{theorem}\label{prop:sitcalc-fo-act}	
  For every possibly open situation calculus formula $\varphi(\vec{x}, s)$ uniform
  in $s$ and with free variables $\vec{x}$ all of object sort, 
  there is a situation calculus formula $\varphi'(\vec{x}, s)$ with no
  occurrence of action terms, again uniform in $s$, such that
$\D_{ca}\models \forall(\varphi(\vec{x}, s) \equiv \varphi'(\vec{x}, s))$.
\end{theorem}
\begin{proofsk}
The proof is by  induction on the structure of the formula $\varphi$.
For $\varphi=F(\vec t,s)$, since $\vec t$ cannot be of sort action, 
$\varphi'=\varphi$.
For $\varphi=A(\vec y)=A'(\vec{y'})$, if $A=A'$, 
let $\varphi'=\vec y=\vec{y'}$, else $\varphi'=\bot$.
For the boolean connectives $\land$ and $\lnot$, the
transformation applies inductively.
%%
If $\varphi=\forall a. \phi(\vec x,a,s)$, 
consider, for every action type $A\in\A$, the formula
$\phi_A(\vec x,s)=\phi(\vec x,A(\vec y),s)$, with 
fresh variables $\vec y$  which do not occur already in  $\phi$,
where $\phi(\vec x,A(\vec y),s)$ is obtained by syntactically 
substituting, in $\phi$, each occurrence of $a$ with $A(\vec y)$. 
Let $\phi'_A$ be a formula, 
existing by induction hypothesis,
with no action terms and such that~$\D_{ca}\models \forall(\phi_A\equiv \phi_A')$, 
and let $\varphi'=\bigwedge_{A\in\A}\phi_A'(\vec x,s)$.
%%
Obviously, $\varphi'$ contains no action term and 
is uniform in $s$.
%%
By considering unique name axioms for actions
and domain closure for action types ($\D_{ca}$),
we easily obtain $\D_{ca}\models \forall(\varphi\equiv\varphi')$.
%%
\begin{comment}
\textbf{GD: notice that some notation now is dropped}
We prove a slightly more general result:
	given a situation calculus formula 
	$\varphi(\vec x,\vec a,s)$  where $\vec x$ ranges over objects,
$\vec a$ over actions, and $s$ over situation terms,
	with $\vec a=\tup{a_1,\ldots,a_\ell}$
	and $\free(\varphi)\subseteq \vec x\cup \vec a\cup\set{s}$,
	for every tuple of action types 
	$\vec A=\tup{A_1,\ldots,A_\ell}$, we show that
	there exists a formula 
	$\varphi_{\vec A}(\vec x,\vec y_1,\ldots,\vec y_\ell,s)$ 
	uniform in $s$, s.t.:
	no action term occurs in $\varphi_{\vec A}$;
	$\const(\varphi_{\vec A})\subseteq\const(\varphi)$; 
	and
	for every $\vec o_x\in\Delta^{\card{\vec x}}$,
	$\vec o_{y_1}\in\Delta^{\card{\vec y_1}},\ldots,
	\vec o_{y_\ell}\in\Delta^{\card{\vec y_\ell}}$,
	and $\bar s\in \S$,
	$\M\models\varphi(\vec o_x,A_1(\vec o_{y_1}),\ldots,A_\ell(\vec o_{y_\ell}),\bar s)\Lra
	\M\models\varphi_{\vec A}(\vec o_x,\vec o_{y_1},\ldots,\vec o_{y_\ell},\bar s)$.
%%
	The proof is by induction on the structure of $\varphi(\vec x,\vec a,s)$.
	Here, we show how to obtain $\varphi_{\vec A}$ from $\varphi$. 
	
	If $\varphi$ contains no action terms, $\varphi_{\vec A}=\varphi$.
	%%
	For $\varphi(\vec x,\vec a,s)= a=A(\vec t)$, 
	let $\vec A=\tup{A_1}$.
	If $A=A_1$, then
	$\varphi_{\vec A}=\bigwedge_{i=1}^{\card{\vec t}} y_{1i}=t_i$,
	else $\varphi_{\vec A}=\bot$.
	%%
	If $\varphi(\vec x,\vec a,s)= \lnot\phi$,
	$\varphi_{\vec A}= \lnot\phi_{\vec A}$.
	%%
	If $\varphi(\vec x,\vec a,s)= \phi(\vec x_\phi,\vec a_\phi,s)\land 
	\phi(\vec x_\psi,\vec a_\psi,s)$, with $\vec x=\vec x_\phi\cup \vec x_\psi$
	and $\vec a=\vec a_\phi\cup \vec a_\psi$, 
	for $\vec A=\tup{A_1,\ldots,A_\ell}$, consider 
	the projections of $\vec A$ on $\vec a_\phi$ and $\vec a_\psi$, 
	respectively $\vec A_\phi$ and $\vec A_\psi$, and let 
	$\varphi_{\vec A}= \phi_{\vec A_{\phi}}\land \psi_{\vec A_{\psi}}$.
	%%
	If $\varphi(\vec x,\vec a,s)= \forall z \phi(\vec x,z,\vec a,s)$,
	given $\vec A=\tup{A_1,\ldots,A_\ell}$, 
	derive, from $\phi$, 
	$\phi_{\vec A}(\vec x,z,\vec y_1,\ldots,\vec y_\ell, s)$. Then, let
	$\varphi_{\vec A}=\forall z\phi_{\vec A}(\vec x,z,\vec y_1,\ldots,,\vec y_\ell,s)$.
	%%
	
	For $\varphi(\vec x,\vec a,s)= \forall a\phi(\vec x,\vec a,a,s)$, 
	it can be proven that $\varphi$ is equivalent to 
	$\varphi(\vec x,\vec a,s)=\bigwedge_{A\in\A}\forall \vec y \phi^{A}(\vec x,\vec a,\vec y,s)$,
	where $\phi^{A}\doteq\phi[a/A(\vec y)]$.
	%%
	Given $\vec A=\tup{A_1,\ldots,A_\ell}$, 
	for every $A\in\A$, consider $\phi^A$, and derive 
	$\phi^A_{\vec A}(\vec x,\vec y_1,\ldots,\vec y_\ell,\vec y,s)$.
	Let $\varphi_{\vec A}=\bigwedge_{A(\vec y)\in\A}
	\forall \vec y\phi^A_{\vec A}(\vec x,\vec y_1,\ldots,\vec y_\ell,\vec y,s)$.
	%%
	\end{comment}
	\begin{comment}
	%%Complete proof
	By induction on the structure of $\varphi(\vec x,\vec a,s)$.
	Let $\A$ be the (finite) set of action types.
	
	If $\varphi$ contains no action terms, let
	$\varphi_{\vec A}=\varphi$.
	
	For $\varphi(\vec x,\vec a,s)= a=A(\vec t)$ (i.e., $\ell=1$), 
	where $\vec t$ is a tuple  of terms s.t.~$\vec x\subseteq \vec t$, 
	let $\vec A=\tup{A_1}$.
	If $A=A_1$, then
	$\varphi_{\vec A}=\bigwedge_{i=1}^{\card{\vec t}} y_{1i}=t_i$,
	else $\varphi_{\vec A}=\bot$.
	%%
	
	If $\varphi(\vec x,\vec a,s)= \lnot\phi$,
	let $\varphi_{\vec A}(\vec x,\vec a,s)= \lnot\phi_{\vec A}$.
	
	If $\varphi(\vec x,\vec a,s)= \phi(\vec x_\phi,\vec a_\phi,s)\land 
	\phi(\vec x_\psi,\vec a_\psi,s)$, with $\vec x=\vec x_\phi\cup \vec x_\psi$
	and $\vec a=\vec a_\phi\cup \vec a_\psi$, 
	for $\vec A=\tup{A_1,\ldots,A_\ell}$, consider 
	the projections of $\vec A$ on $\vec a_\phi$ and $\vec a_\psi$, 
	respectively $\vec A_\phi$ and $\vec A_\psi$, and let 
	$\varphi_{\vec A}(\vec x,\vec a,s)= \phi_{\vec A_{\phi}}\land \psi_{\vec A_{\psi}}$.
	
	The thesis can be easily proven in all the above cases.
	
	For $\varphi(\vec x,\vec a,s)= \forall z \phi(\vec x,z,\vec a,s)$,
	assume, w.l.o.g., $\free(\phi)=\free(\varphi)\cup\set{z}$
	(if $z\notin\free(\phi)$, remove the quantification and 
	consider the appropriate case for the resulting $\varphi$).
	Obviously, $\const(\varphi)=\const(\phi)$.
	%%
	Given $\vec A=\tup{A_1,\ldots,A_\ell}$, 
	by induction hypothesis,
	there exists an action-term-free formula
	$\phi_{\vec A}(\vec x,z,\vec y_1,\ldots,\vec y_\ell, s)$
	s.t.~$\const(\phi_{\vec A})\subseteq\const(\phi)$, 
	and for every
	$\vec o_x,o_z,\vec o_{y_1},\vec o_{y_\ell},\bar s$  (of appropriate sort and length),
	$\M\models\phi(\vec o_x,o_z,A(\vec o_{y_1}),\ldots,A(\vec o_{y_\ell}),\bar s)\Lra
	\M\models\phi_{\vec A}(\vec o_x,o_z,\vec o_{y_1},\ldots,\vec o_{y_\ell},\bar s)$.
	%%
	This, in turn, implies that
	%%for every 
	%%$\vec o_x,\vec o_{y_1},\ldots,\vec o_{y_\ell},s$,
	%%as above,
	$\M\models\forall z\phi(\vec o_x,z,A(\vec o_{y_1}),\ldots,A(\vec o_{y_\ell}),\bar s)\Lra
	\M\models\forall z\phi_{\vec A}(\vec o_x,z,\vec o_{y_1},\ldots,\vec o_{y_\ell},\bar s)$.
	%%
	Thus, the thesis follows, by defining
	$\varphi_{\vec A}=\forall z\phi_{\vec A}(\vec x,z,\vec y_1,\ldots,,\vec y_\ell,s)$,
	and observing that $\const(\varphi_{\vec A})=\const(\phi_{\vec A})\subseteq\const(\phi)=\const(\varphi)$.
	
	For $\varphi(\vec x,\vec a,s)= \forall a\phi(\vec x,\vec a,a,s)$, 
	since we have domain closure on the set of actions, 
	and being the set of action types finite, 
	$\varphi$ is equivalent to 
	$\varphi(\vec x,\vec a,s)=\bigwedge_{A\in\A}\forall \vec y \phi^{A}(\vec x,\vec a,\vec y,s)$,
	where $\phi^{A}\doteq\phi[a/A(\vec y)]$.
	%%is obtained from $\phi(\vec x,\vec a,a,s)$, by
	%%replacing the variable $a$ with the action term $A(\vec y)$.
	%%
	Now, by induction hypothesis, given $\vec A=\tup{A_1,\ldots,A_\ell}$, 
	for every $A\in\A$ and corresponding $\phi^A$, 
	there exists an action-term-free $\phi^A_{\vec A}(\vec x,\vec y_1,\ldots,\vec y_\ell,\vec y,s)$ 
	s.t.~for every $\vec o_x,\vec o_{y_1},\vec o_{y_\ell},\vec o_y,\bar s$,
	$\M\models\phi(\vec o_x,A_1(\vec o_{y_1}),\ldots,A_\ell(\vec o_{y_\ell}),A(\vec o_y),\bar s)\Lra
	\M\models\phi^{A}_{\vec A}(\vec o_x,\vec o_{y_1},\ldots,\vec o_{y_\ell},\vec o_y,\bar s)$.
	%%
	This implies that, for every $A\in\A$,
	$\M\models\forall \vec y\phi(\vec o_x,A_1(\vec o_{y_1}),\ldots,A_\ell(\vec o_{y_\ell}),A(\vec y),\bar s)\Lra
	\M\models\forall \vec y\phi^A_{\vec A}(\vec o_x,\vec o_{y_1},\ldots,\vec o_{y_\ell},\vec y,\bar s)$.
	%%
	Observe that even though
	$\const(\phi^A_{\vec A})\subseteq\const(\phi^A)=\const(\phi)\cup\bigcup_{A\in\A} A$, 
	because $\phi^A_{\vec A}$ contains no action term, 
	necessarily $\const(\phi^A_{\vec A})\subseteq\const(\phi)$.
	%%
	Thus, the thesis follows by defining $\varphi_{\vec A}(\vec x,\vec a,s)=\bigwedge_{A(\vec y)\in\A}
	\forall \vec y\phi^A_{\vec A}(\vec x,\vec y_1,\ldots,\vec y_\ell,\vec y,s)$.
	%%
	\end{comment}
\end{proofsk}

Next we show that in a model of the action theory $\D$, the evaluation
in a situation $s$ of a uniform situation calculus formula depends
only on the extensions of the fluents in $s$. This gives us a way of
interpreting directly situation suppressed formulas. By 
Th.~\ref{prop:sitcalc-fo-act} above, without loss of generality, we can
concentrate on formulas where no action terms occur.

In fact, the action theory $\D$, which has complete information on the
initial situation, has essentially one model $\M$ whose object domain is
$\N$. However, we will consider parametric variants $\M_\Delta$ of
$\M$ where we vary the object domain allowing it to be a subset $\Delta$
of $\N$ including the (finite) set $C$ of all constants occurring in 
$\D_{poss}\cup \D_{ssa}\cup \D_0$.
We have the following result for this kind of models:

\begin{theorem}\label{prop:sitcalc-fo}
  Let $\M_\Delta$ be a model of $\D$ with object domain $\Delta$
  and situation domain $\S$, and $v$ an individual variable valuation.
  Let $I_{v(s)}=\tup{\Delta^{I_{v(s)}},\cdot^{I_{v(s)}}}$ be the interpretation
  s.t.~$\Delta^{I_{v(s)}}=\Delta$ and $F^{I_{v(s)}}=\set{\vec u\mid \M_\Delta,v\models F(\vec
    u,s)}$ for every fluents $F\in\F$.  Then for every situation calculus
  formula uniform in $s$, $\varphi(s)$, where no action term occurs,
  with corresponding situation suppressed formula $\varphi$, we
  have:
\[\M_\Delta,v\models \varphi(s) \mbox{ iff } I_{v(s)},v\models \varphi.\] 
\end{theorem}
\begin{proofsk}
	Since no action terms occur in $\varphi$
	and it is uniform in $s$, 
	the evaluation of $\varphi$ depends only on the interpretation of each fluent
	in $s$, and on the individuals in $\Delta$, i.e., on $I_{v(s)}$.
\end{proofsk}

With these two results in place, we can better understand the
expressive capabilities of our verification logic $\mu\L$. First we
observe that by Th.~\ref{prop:sitcalc-fo-act} we can disallow the
occurrence of action terms in $\mu\L$ formulas.  Moreover,  we next
show that, without loss of generality, $\mu\L$ formulas can be
interpreted over suitable transition systems, which abstract away
aspects of situation calculus models that are irrelevant wrt $\mu\L$.


A {\em transition system} (TS) (over the situation suppressed fluents of $\D$) is a tuple 
$T=\tup{\Delta,Q,q_0,\ra,L}$, where:
%\begin{inparaenum}
\begin{itemize}\itemsep=0pt
	\item $\Delta$ is the {\em object domain};
	\item $Q$ is the {\em set of states};
	\item $q_0\in Q$ is the {\em initial state};
	\item $\ra\subseteq Q\times Q$ is the {\em transition relation}; and
	\item $L:Q\mapsto Int^\F_\Delta$ is the {\em labeling function} associating each state $q$ with an FO interpretation $I_q=(\Delta,\cdot^\I_q)$ assigning an extension to situation suppressed fluents in $\D$.
\end{itemize}
%\end{inparaenum}

We can interpret $\mu\L$ formulae over TSs. In particular given a TS
$T=\tup{\Delta,Q,q_0,\ra,L}$, we introduce a predicate variable
valuation $\V$, i.e., a mapping from predicate variables $Z$ to
subsets of $Q$, and we define the \emph{extension function}
$\MODAT{\cdot}$, which maps $\mu\L$ formulae to subsets of $Q$ as
follows:
\[\begin{array}{lcl}
\MODAT{\varphi} &= & \{q \in Q\mid I_q\models \varphi \}\\
\MODAT{\lnot \Phi} &= & Q - \MODAT{\Phi} \\
\MODAT{\Phi_1 \land \Phi_2} &= &\MODAT{\Phi_1}\cap\MODAT{\Phi_2}\\
\MODAT{\DIAM{\Phi}} &= & \{q \in Q\mid\exists q' . q\ra q'\land q' \in \MODAT{\Phi}\} \\
\MODAT{Z} &= & \V(Z)\\
\MODAT{\mu Z.\Phi} &= & \bigcap\{\E\subseteq Q \mid \MODATZ{\Phi}{[Z/\E]}
\subseteq \E \}%\\
\end{array}
\]

Among the various TSs, we are interested in those induced by models of
the action theory $\D$.
%%
Consider a model $\M_\Delta$ of $\D$ with object domain $\Delta$ and situation domain $\S$.
%%
The TS {\em induced by $\M_\Delta$}
is the labelled TS \mbox{$T=\tup{\Delta,Q,q_0,\ra,L}$}, s.t.:
%\begin{inparaenum}
\begin{itemize}\itemsep=0pt
	\item $Q=\S$ is the set of {\em possible states}, 
		each corresponding to a distinct executable $\D$-situation;
	\item $q_0=S_0\in Q$ is the {\em initial state}, 
		with $S_0$ the initial situation of $\D$;
	\item ${\ra}\subseteq Q\times Q$ is the {\em transition relation}
		s.t.~$q\ra q'$ iff there exists some $a$ s.t.~$q'=do^{\M_\Delta}(a,q)$ and
		$(a,q)\in\Poss^{\M_\Delta}$; and
	\item $L: Q\mapsto Int^\F_\Delta$ 
		is the {\em labeling function} 
		associating each state/situation $q$ with an FO interpretation $I=L(q)$ s.t.\
		$F^I=\set{\vec o\mid \M_\Delta\models F(\vec o, q)}$, for every situation suppressed fluent in $\D$.
\end{itemize}
%\end{inparaenum}
%%

\begin{theorem}\label{th:InducedTS}
  Let $\D$ be an action theory, $\M_\Delta$  a model of $\D$ with object domain $\Delta$ and
  situation domain $\S$, and $T$ the TS induced by $\M_\Delta$.
  Then for every $\mu\L$ formula $\Phi$ (with no occurrence of action terms) we have that:
\[(\Phi)^{\M_\Delta}_\V=\MODAT{\Phi}\] 
\end{theorem}
\begin{proofsk}
  By induction on the structure of the formula, exploiting
  Th.~\ref{prop:sitcalc-fo} for the base FO case.
\end{proofsk}
Notice that for $\Delta=\N$ we get \emph{the} ``standard'' model of $\D$.

The main advantage of introducing TSs is that we can
exploit the classical bisimulation invariance results for the
$\mu$-calculus which say that two bisimilar TSs satisfy exactly the
same $\mu$-calculus formulas, see e.g.~\cite{Stirling2001:Modal}. This
implies that TSs that are bisimilar to the one induced by a situation
calculus model satisfy the same formulas, even if their transition
relation is not a tree structure induced by the situation tree. We do not
present the classical bisimulation here. Instead, we introduce below
the weaker notion of active-domain bisimulation, which allows us to
consider bisimilar even TSs that have different object domains.


\begin{comment}
\subsection{Preliminary Notions}
We start by fixing the notation used throughout the proof.
%%
We denote the (countable) set of standard names as $\N$.
For a fixed action theory $\D$, we define 
the finite set of  constants occurring in $\D_{poss}\cup \D_{ssa}\cup \D_0$ %% $\D$
(including those in $\D_0$) as $C\subseteq\N$,
and the set $\F$ of relational fluent symbols of $\D$.
%%

By $\L_\D$ we mean the language of FO formulas
including all the action-free, situation-suppressed 
situation calculus formulas over $\D$.
%%
%%is inductively defined as follows:
%%$$\varphi ::= F(t_1,\ldots, t_n)\mid t=t'\mid \lnot\varphi\mid \varphi\land\varphi\mid \forall x\varphi,$$
%%where $F\in\F$ and $t,t',t_i$ are terms, i.e., variables or constant symbols from $C$.
%%
%%Free and bound variables, and the boolean 
%%connectives  $\exists$, $\ra$, and $\wedge$, 
%%are defined in the standard way. We use $=$ also for syntactic equivalence
%%among formulas.
W.l.o.g., we assume that no variable is quantified 
more than once in a formula (otherwise, just rename the variables).
%%
For a formula $\varphi$, $\vars(\varphi)$,
$\const(\varphi)$, and $\free(\varphi)$ denote,
respectively, the set of variables, constants, and
free variables occurring in $\varphi$.
%%A {\em sentence} $\varphi$ is a formula s.t.~$\free(\varphi)=\emptyset$.
%%
By slight abuse of notation, we 
consider tuples as sets. 
Thus, we can write 
$x\in\vec x$, to refer to the generic 
$\vec x$-component $x$.
%%
Unless differently stated, $\varphi(\vec x)$ 
expresses the fact that $\free(\varphi)=\vec x$.

\textbf{FP: standard? We interpret relational symbols as finite relations!}
The semantics of $\L_\D$ formulas is defined as standard, 
in terms of interpretations $I=\tup{\Delta^I,\cdot^I}$
associating each symbol $F\in\F$,
of appropriate cardinality, 
with a finite relation $F^I$ over the object domain. 
$Int^\F_\Delta$ denotes the set of all 
interpretations of $\F$ over an object domain $\Delta$.
%%
%%An {\em interpretation} of $\F$ 
%%over (the interpretation domain) $\Delta^I$
%%is a pair $I=\tup{\Delta^I,\cdot^I}$, 
%%where $C\subseteq\Delta^I\subseteq \N$, and 
%%$\cdot^I$ is a mapping associating: 
%%each constant symbol $c\in C$ with a constant $c^I=c$; and
%%each relational fluent symbol $F\in\F$ with a finite
%%relation $F^I\subseteq (\Delta^I)^a$, where $a$ is the arity of $F$.
%%
%%Given an interpretation $I$, 
%%a formula $\varphi(\vec x)$,
%%and a tuple $\vec o\in\N^{\card{\vec x}}$,  
%%we say that $I$ {\em satisfies} 
%%$\varphi(\vec x)$ under $\vec o$, 
%%written $(I,\vec o)\models\varphi$,
%%or $I\models\varphi(\vec o)$ for short, if either:
%%%%
%%\begin{inparaenum}
%%	\item $\varphi= F(\vec t)$, 
%%		and $\tup{\omega_1,\ldots,\omega_{\card{\vec t}}}\in F^I$, 
%%		where $\omega_i=t_i^I$, if $t_i\in C$, and
%%		$\omega_i=o_j$, if $t_i$ is $x_j$; or
%%	\item $\varphi= t_1=t_2$,
%%		and $\omega_1$ is $\omega_2$, where 
%%		$\omega_i=t_i^I$, if $t_i\in C$, and 
%%		$\omega_i=o_j$, if $t_i$ is $x_j$; or
%%	\item $\varphi= \forall x\phi$,
%%		and for every $o\in \Delta^I$, 
%%		$(I,\vec{o'})\models\phi$,
%%		where $\card{\vec{o'}}=\card{\vec o}+1$,
%%		for $i=1,\ldots,\card{\vec o}$, $o'_i=o_i$, and
%%		$o'_\ell=o$, for $\ell=\card{\vec{o'}}$; or
%%	\item $\varphi= \lnot \phi$, and 
%%		$(I,\vec{o})\not\models\phi$; or
%%	\item $\varphi= \phi(\vec x_\phi)\land\psi(\vec x_\psi)$, and
%%		$(I,\vec{o_\phi})\models\phi$
%%		and 
%%		$(I,\vec{o_\psi})\models\psi$,
%%		for $\vec o_\phi$ (resp., $o_\psi$) 
%%		s.t.~$o_{\phi i}=o_j$ ($o_{\psi i}=o_j$),
%%		if $x_{\phi i}$ ($x_{\psi i}$) is $x_j$.
%%\end{inparaenum}
\end{comment}


\subsection{Active-Domain Isomorphism and Bisimulation}
We now define the notion of active-domain isomorphic 
interpretations, i.e., interpretations 
with the same relational structure but possibly renamed objects,
and present some basic results that are fundamental to perform 
the abstraction step.  Then, based on the notion of 
active-domain isomorphism, we devise that of active-domain 
bisimulation.

We fix an action theory $\D$. 
% We denote by $C$ the finite 
% set of object constants occurring in $\D$ (including those in $\D_0$),
% and  with $\F$ the set of (relational)
% fluents of $\D$.
%%
With a slight abuse of notation we use $\F$ to denote both the set of fluents and their corresponding situation suppressed version.
%%
By $\L_\D$ we mean the language of FO formulas built
from the situation suppressed fluents in $\F$ and equality.
Notice that these formulas are the FO formulas in $\mu\L$ 
(once action terms have been removed).
%%
The {\em active domain} of an interpretation $I$, $\adom(I)$, 
is the set of all objects occurring in some $F^I$ ($F\in\F$) or in the set $C$ of constants occurring in 
$\D_{poss}\cup \D_{ssa}\cup \D_0$.
%%$\D$.
%%
In what follows, $I$ and $J$ denote two interpretations 
of $\F$, $\varphi(\vec x)\in\L_\D$, and $\card{\vec x}=\ell$.
%%

We say that $I$ and $J$
are {\em active-domain isomorphic},
written $I\sim J$, if 
there exists a bijection $i:\adom(I)\mapsto \adom(J)$ 
%%
s.t.~$i(c^I)=c^J$ and   $\vec o\in F^I$ iff $i(\vec o)\in F^J$.
%%
The bijection $i$ is also called an {\em active-domain isomorphism},  
or {\em A-isomorphism} for short, from $I$ to $J$. 
%%
Obviously, $i$ is invertible, and $i^{-1}$ is an A-isomorphism
from $J$ to $I$. 
%%
%%Thus, it can be easily seen that $\sim$ is an equivalence relation.

In addition we define a similar, though stronger, relation among tuples.
%%
Fix an (arbitrary) relational fluent name $P$ not occurring in $\F$,
and define, for a tuple $\vec o\in(\Delta^I)^\ell$,
$I+\vec o$ as the interpretation
$I'$ over the schema $\F\uplus\set{P/\ell}$, s.t.:
\begin{inparaenum}
	\item $\Delta^{I'}=\Delta^I$;
	\item for every $F\in\F$, $F^I=F^{I'}$; and
	\item $P^{I'}=\set{\vec o}$.
\end{inparaenum}
%%
Essentially, $I'$ (i.e., $I+\vec o$) is analogous to $I$ except for the additional 
relation symbol $P$ of arity $\ell$, interpreted as the tuple $\vec o$.
%%
We say that two tuples 
$\vec o_1\in(\Delta^I)^\ell$ and
$\vec o_2\in(\Delta^J)^\ell$
are {\em equivalent} 
for $I$ and $J$,
if $I+\vec o_1\sim J+\vec o_2$.
%%
Informally, two tuples are equivalent if ``adding''
them to A-isomorphic interpretations 
results again in A-isomorphic interpretations. 
%%

The following results formalize the intuition that 
when a formula $\varphi$ is evaluated 
against A-isomorphic interpretations,
equivalent tuples play the same role.
%%
%%To see this, let $I\sim J$, and $N=\card{\adom(I)}=\card{\adom(J)}$.
%%
\begin{theorem}\label{prop:iso-eq}
	Let $I\sim J$, and $N=\card{\adom(I)}=\card{\adom(J)}$.
If  
	%%$I\sim J$, and 
%	$\card{\Delta^I}=\card{\Delta^J}$ or 
	both $\card{\Delta^I}$ and $\card{\Delta^J}$ are  ${} \geq N+\card{\vars(\varphi)}$, 
	then for every formula $\varphi(\vec{x})\in \L_\D$ and every two equivalent tuples 
	$\vec o_I\in(\Delta^I)^\ell$ and 
	$\vec o_J\in(\Delta^J)^\ell$, 
	$I\models\varphi(\vec o_I)\Lra J\models\varphi(\vec o_J)$.
\end{theorem}
%%
\begin{proofsk}
	By induction on the structure of $\varphi$.
	\begin{comment}
	Let $i:\adom(I+\vec o_I)\mapsto \adom(J+\vec o_J)$ be an A-isomorphism 
	witnessing that $\vec o_I$ and $\vec o_J$ are equivalent, and observe that
	$\vec o_J=i(\vec o_I)$.
	%%
	Using $i$, the proof consists of showing that, for each case, 
	$I\models\varphi(\vec o_I)\Ra J\models\varphi(\vec o_J)$. 

	The cases of $\varphi(\vec x)= F(\vec t)$, $\varphi(\vec x)= t=t'$,
	and $\varphi(\vec x)= \phi(\vec x_\phi)\land\psi(\vec x_\psi)$ are 
	proven directly.
	The cases of $\varphi(\vec x)= \lnot\phi(\vec x)$ and 
	$\varphi(\vec x)= \forall x\phi(\vec x,x)$ 
	are proven by contradiction.

	The opposite directions are proven analogously, by observing 
	that $\sim$ is symmetric, by swapping 
	$I$ and $J$, and by replacing $i$ with its inverse $i^{-1}$.
	\end{comment}
	%%
	\begin{comment}
	%%Complete proof
	The proof is by induction on the structure of $\varphi$.
	%%
	Let $i:\adom(I+\vec o_I)\mapsto \adom(J+\vec o_J)$ be an A-isomorphism 
	witnessing that $\vec o_I$ and $\vec o_J$ are equivalent, and observe that
	$\vec o_J=i(\vec o_I)$.
	%%
	For each case, we prove 
	that  $I\models\varphi(\vec o_I)\Ra J\models\varphi(\vec o_J)$. 
	The opposite directions are proven analogously, by observing 
	that $\sim$ is symmetric, by swapping 
	$I$ and $J$, and by replacing $i$ with its inverse $i^{-1}$.
	%%
	
	For $\varphi(\vec x)= F(\vec t)$, where $\vec t$ is a tuple of terms 
	s.t.~$\vec x\subseteq \vec t$, 
	define $\vec \omega_I\in(\Delta^I)^{\card{\vec t}}$
	s.t.~$\omega_{Ii}=t_i^I$, if $t_i\in C$, and 
	$\omega_{Ii}=o_{Ij}$, if $t_i$ is $x_j$.
	%%
	By definition of satisfaction, 
	$I\models\varphi(\vec o_I)$ implies
	$\vec\omega_I\in F^I$.
	%%
	Thus, $i$ being an A-isomorphism, for 
	$\vec \omega_J=i(\vec \omega_I)$, $\vec \omega_J\in F^J$. 
	%%Thus $J\models \varphi(\vec \omega_J)$.
	%%
	But because $i(c^I)=c^J=c$,
	$\const(\varphi)\subseteq C$,
	and $\vec o_J=i(\vec o_I)$, 
	it can be seen that $\vec \omega_J$ is
	s.t.~$\omega_{Ji}=t_i^J$, if $t_i\in C$, and 
	$\omega_{Ji}=o_{Jj}$, if $t_i$ is $x_j$.
	But then, by definition of satisfaction,
	$J\models \varphi(\vec o_J)$.
	
	For $\varphi(\vec x)= t=t'$, either both $t$ and $t'$ are variables, 
	or only one does (and the other is a constant). 
	W.l.o.g., assume $t$ is $x_1$.
	If $t'$ is $x_2$  (i.e., $\vec x=\tup{x_1,x_2}$), 
	and $I\models \varphi(\vec o_I)$, 
	with $\vec o_I=\tup{o_{I,1},o_{I,2}}$, 
	then $o_{I,1}=o_{I,2}$.
	Thus, $i(o_{I,1})=i(o_{I,2})$, and 
	for $\vec {o_J}=\tup{i(o_{I,1}),i(o_{I,2})}$, 
	$J\models \varphi(\vec {o_J})$.
	%%
	If $t'$ is a constant (thus $\vec x=\tup{x_1}$), 
	necessarily $t'\in\const(\varphi)$.
	%%
	Moreover, if $I\models \varphi(\vec o_I)$, 
	$\vec o_I=\tup{o_{I,1}}=\tup{t'^I}$. 
	But $i(t'^I)=t'$, as $i(c^I)=c^J=c$, 
	for $c\in\const(\varphi)\subseteq C$.
	%%
	Thus, $\vec{o_J}=i(\vec o_I)=i(\tup{t'^I})=\tup{t'^I}$, 
	therefore $J\models \varphi(\vec o_J)$.
	
	For $\varphi(\vec x)= \lnot\phi(\vec x)$, 
	assume by contradiction that
	$I\models\varphi(\vec{o_I})$
	and
	$J\not\models\varphi(\vec{o_J})$.
	%%
	Since the latter is equivalent to
	$J\models\phi(\vec{o_J})$,
	%%
	observing that $\sim$ is symmetric, 
	by induction hypothesis,
	$I\models\phi(\vec o_I)$, that is,
	$I\not\models\varphi(\vec o_I)$. 
	Contradiction.
	
	For $\varphi(\vec x)= \phi(\vec x_\phi)\land\psi(\vec x_\psi)$ 
	($\vec x=\vec x_\phi\cup\vec x_\psi$),
	consider $o_I$ s.t.~$I\models\varphi(\vec o_I)$, and 
	let $\vec o_{I\phi}$ and $\vec o_{I\psi}$ be the projections of 
	$\vec o_I$ on $\vec x_\phi$ and $\vec x_\psi$, respectively.
	%%
	Obviously, $I\models\phi(\vec o_{I\phi})$
	and $I\models\psi(\vec o_{I\psi})$.
	%%
	Considering $\vec o_J=i(\vec o_I)$,
	it can be seen that the projections of $\vec o_J$
	on $\vec x_\phi$ and $\vec x_\psi$, i.e.,
	$\vec o_{J\phi}$ and $\vec o_{J\psi}$, are 
	s.t.~$\vec o_{J\phi}=i(\vec o_{I\phi})$, 
	and $\vec o_{J\psi}=i(\vec o_{I\psi})$. 
	%%
	Moreover, it can be proven that
	$\vec o_{J\phi}$ and $\vec o_{I\phi}$ are equivalent,
	as well as  $\vec o_{J\psi}$ and $\vec o_{I\psi}$.
	%%
	Thus, by induction hypothesis, 
	$J\models\phi(\vec o_{J\phi})$
	and $J\models\psi(\vec o_{J\psi})$.
	Therefore, $J\models\varphi(\vec o_J)$.
	
	For $\varphi(\vec x)= \forall x\phi(\vec x,x)$, 
	assume by contradiction that 
	$I\models\forall x\phi(\vec o_I,x)$ but
	$J\not\models\forall x\phi(\vec o_J,x)$.
	%%
	Thus, there exists $o_J\in\Delta^J$ 
	s.t.~$J\not\models\phi(\vec o_J,o_J)$, i.e.,
	$J\models\lnot\phi(\vec o_J,o_J)$.
	%%
	Now define a function $j:\adom(J)\cup\vec o_J\cup\set{o_J}\mapsto \Delta^I$ 
	as follows: 
	if $o_J\in\adom(J)\cup\vec o_J$, then $j\doteq i^{-1}$;
	otherwise, $j$ is an extensions of $i^{-1}$ to $o_J$ that is injective.
	%%
	We need to prove that such a $j$ exists in the latter case.
	If $\card{\Delta^I}=\card{\Delta^J}$, this is straightforward.
	If $\card{\Delta^I},\card{\Delta^J}\geq N+\card{\vars(\varphi)}$,
	observe that, because $\free(\phi)\subseteq\vars(\varphi)$,
	then $\card{\vars(\varphi)}\geq\card{\vec x}+\card{\set{x}}=\card{\vec o_J}+1=\card{\vec o_I}+1$.
	Thus, if $\card{\Delta^I},\card{\Delta^J}\geq N+\card{\vars(\varphi)}$,
	in particular $\card{\Delta^I}\geq N+\card{\vec o_J}+1$, which is 
	sufficient in order for an injective $j$ as above to exist. 
	%%
	Obviously, the function 
	$j':\adom(J)\cup\vec o_J\cup\set{o_J}\mapsto \adom(I)\cup\vec o_I\cup\set{o_I}$
	s.t.~$j'=j|_{\adom(J)\cup\vec o_J\cup\set{o_J}}$ is a bijection.
	%%
	Define
	$\vec u_I=\tup{o_{I1},\ldots,o_{I\ell},j(o_J)}$ 
	and 
	$\vec u_J=\tup{o_{J1},\ldots,o_{J\ell},o_J}$, and
	observe that, by the way $j'$ (and $j$) is defined,
	$j'$ is an A-isomorphism from $J+\vec u_J$ to $I+\vec u_I$.
	%%
	Thus, $\vec u_I$ and $\vec u_J$  are equivalent.
	%%
	But then, by induction hypothesis,
	$I\models\lnot\phi(\vec o_I,j(o_J))$, i.e.,
	$I\not\models\forall x\phi(\vec o_I,x)$. Contradiction.
	%%
	\end{comment}
\end{proofsk}
%%
This theorem states that, under appropriate cardinality constraints,
the evaluation of a FO formula against an interpretation and a variable
assignment,  depends 
only on the relational structure of the data in the 
interpretation and the assignment. 
Thus, for our verification purposes, $I$ and $\vec o_1$
can be equivalently replaced by $J$ and $\vec o_2$.
%%
Observe that if $\card{\Delta^I}=\card{\Delta^J}$ then independently 
from the cardinality, the thesis of the theorem trivially holds, as the 
A-isomorphism induces a standard  isomorphism between the two interpretations.
%%
This result generalizes to the interpretation of open FO formulas
under partial variable assignments, as shown by Th.~\ref{prop:iso-query},
which is, in turn, proven using Lemma~\ref{prop:fin-ans}.

For an interpretation $I$ and an
$\L_\D$ formula $\varphi(\vec x,\vec y)$, 
given $\vec u\in\Delta^{\card{\vec y}}$, we define 
$\varphi(\vec x,\vec u)^I\doteq\set{\vec o\in\Delta^{\card{\vec x}}\mid I\models\varphi(\vec o,\vec u)}$.
%%
Intuitively, $\varphi(\vec x, \vec y)$ can be seen as a sort of parametric query
(i.e., an open formula), with $\vec x$ and $\vec y$ intended to be
output and input parameters respectively.  Moreover $\varphi(\vec
x, \vec u)^I$ can be seen as the result, i.e., the \emph{answer}, of evaluating
$\varphi$ against $I$, with (actual) input parameters $\vec
u$.
%%
\begin{lemma}\label{prop:fin-ans}
Let $I$ be an interpretation and
  %%$I\sim J$, and 
  $\varphi(\vec x)$ be an $\L_\D$ formula. For every
  partition $\vec x=\set{\vec x_1,\vec x_2}$ and tuple $\vec u\in
  (\Delta^I)^{\card{\vec x_2}}$, if $\Delta^I$ is infinite and
  $\varphi(\vec x_1, \vec u)^I$ is finite, then $\varphi(\vec x_1,
  \vec u)^I\subseteq (\adom(I)\cup \vec u)^{\card{\vec x_1}}$.
\end{lemma}
	\begin{proofsk}
		Observing that $I\sim I$ ($\sim$ is reflexive), and
		using Th.~\ref{prop:iso-eq},
		it can be proved 
		that if $\varphi(\vec x_1,\vec u)^I$ contains 
		a tuple $\vec o$ with some object not 
		from $\adom(I)$ or $\vec u$, then it
		contains also all the other
		infinitely many tuples equivalent to $\vec o$. 
		But then $\varphi(\vec x_1, \vec u)^I$ is infinite.
		Contradiction.
	\end{proofsk}
\begin{comment}
%%Complete proof
	\begin{proofsk}
	Firstly observe that $I\sim I$ and, because $\Delta^I$ is infinite,
	$\card{\Delta^I}\geq \card{\adom(I)}+\card{\vars(\varphi)}$.
	Thus, for $J=I$, the hypotheses of  Th.~\ref{prop:iso-eq} hold.
	%%
	Next assume by contradiction that there exists a tuple 
	$\vec o=\tup{o_1,\ldots,o_m}\in\varphi(\vec x_1,\vec u)^I$ s.t.,
	for some $k$, $o_k\notin\adom(I)\cup\vec u$.
	%%
	Consider $o'\in\Delta^I\setminus(\adom(I)\cup\vec o\cup \vec u)$
	(it exists, because $\Delta^I$ is infinite),
	and let $\vec {o'}=\tup{o'_1,\ldots,o'_m}$
	be a tuple obtained from $\vec o$ by 
	replacing each component $o_i$ s.t.~$o_i=o_k$
	with $o'$, and leaving the remaining components unchanged.
	%%
	It can be seen that  $\tup{\vec {o'},\vec u}$ is equivalent to 
	$\tup{\vec o,\vec u}$ (consider the bijection 
	$i:\adom(I)\cup \vec u\cup \vec o\mapsto 
	\adom(I)\cup \vec u\cup (\vec o\setminus\set{o_k})\cup\set{o'}$
	s.t.~$i(o_k)=o'$, and $i(o)=o$, for $o\neq o_k$).
	%%
	Hence, by  Th.~\ref{prop:iso-eq}, 
	$I\models\varphi(\vec {o'},\vec u)$, 
	thus $\vec {o'}\in \varphi(\vec x_1, \vec u)^I$.
	%%
	But since $\Delta^I$ is infinite, 
	there exist infinitely many distinct such $o'$.
	%%
	Thus, $\varphi(x_1,\vec u)^I$ is infinite. Contradiction.
	\end{proofsk}
\end{comment}
%%
\begin{theorem}\label{prop:iso-query}
	Let $I\sim J$ and 
	$\varphi(\vec x)$ be an $\L_\D$ formula. For every partition $\vec x=\set{\vec x_1,\vec x_2}$ 
	and equivalent 
	tuples 
	$\vec u\in (\Delta^I)^{\card{\vec x_2}}$ and 
	$\vec v\in (\Delta^J)^{\card{\vec x_2}}$,
%%Partition $\vec x$ as $\vec x=\set{\vec x_1,\vec x_2}$, and 
%%consider $\varphi(\vec x)=\varphi(\vec x_1, \vec x_2)$.
%%
%%Given two equivalent tuples 
%%$\vec u\in (\Delta^I)^{\card{\vec x_2}}$ and 
%%$\vec v\in (\Delta^J)^{\card{\vec x_2}}$,
%%
if $\Delta^I$ is infinite, 
$\card{\Delta^J}\geq N+\card{\vars(\varphi)}$
($N=\card{\adom(I)}=\card{\adom(J)}$),
and $\varphi(x_1,\vec u)^I$ is finite, 
then for every A-isomorphism 
$i:\adom(I)\cup\vec u\mapsto \adom(J)\cup\vec v$ witnessing that 
$I+ \vec u\sim J+\vec v$,
$\vec o\in\varphi(x_1,\vec u)^I$ iff $i(\vec o)\in\varphi(x_1,\vec v)^J$.
\end{theorem}
%%
\begin{proofsk}
	Both directions come as a consequence of  
	Lemma~\ref{prop:fin-ans} and Th.~\ref{prop:iso-eq}.
	The only-if part is straightforward. The 
	if-part requires additional care to prove that the 
	A-isomorphism witnessing $I\sim J$ can be inverted 
	on the elements  occurring in $\varphi(x_1,\vec v)^J$.
	%%
	\begin{comment}
		Let $i$ be an A-isomorphism witnessing $I+\vec u\sim J+\vec v$.
		For the only-if part, consider $\vec o\in\varphi(x_1,\vec u)^I$.
		By Lemma~\ref{prop:fin-ans}, 
		$\varphi(x_1,\vec u)^I\subseteq(\adom(I)\cup \vec u)^{\card{\vec x_1}}$,
		so $\vec o\in(\adom(I)\cup \vec u)^{\card{\vec x_1}}$, 
		thus $i(\vec o)$ is defined.
		%%
		Since, by hypothesis, $\vec v=i(\vec u)$, 
		it can be seen that $\tup{\vec o, \vec u}$ is equivalent to $i(\tup{\vec o, \vec u})=\tup{i(\vec o), \vec v}$.
		%%
		Therefore, 
		because $\vec o\in\varphi(x_1,\vec u)^I\Ra I\models\varphi(\vec o,\vec u)$, 
		by Th.~\ref{prop:iso-eq}, 
		$J\models\varphi(i(\vec o),\vec v)$. 
		Thus, again by Th.~\ref{prop:iso-eq}, $i(\vec o)\in\varphi(x_1,\vec v)^J$.
		
		For the if-part, consider $\vec o\in\varphi(\vec x_1,\vec v)^J$.
		%%
		It is necessarily the case that 
		$\vec o\in(\adom(J)\cup \vec v)^{\card{\vec x_1}}$. 
		To see it, assume by contradiction this is not the case.
		%%
		Then, there exists some component $o_k$ of $\vec o$ 
		s.t.~$o_k\notin\adom(J)\cup \vec v$.
		%%
		Consider an injective function 
		$g:\adom(J)\cup \vec v\cup \vec o\mapsto \Delta^I$ 
		that extends $i^{-1}$ to 
		$\vec o\setminus(\adom(J)\cup \vec v)$.
		%%
		Such a $g$ exists, because
		$\vec o\setminus (\adom(J)\cup \vec v)$ is finite, 
		while $\Delta^I\setminus(\adom(I)\cup \vec u)$ is infinite. 
		%%
		Obviously, by definition of $i$, $g(\vec v)=i^{-1}(\vec v)=\vec u$.
		%%
		Moreover, it can be seen that 
		$\tup{\vec o,\vec v}$ is equivalent to 
		$g(\tup{\vec o,\vec v})=\tup{g(\vec o),\vec u}$
		(a witness of this is the bijection 
		$g':\adom(J)\cup \vec v\cup \vec o\mapsto \adom(I)\cup \vec u\cup g(\vec o)$
		s.t.~$g'=g$).
		%%
		In addition, because $g$ is injective and a proper extension  
		of $i^{-1}$, which is a bijection, 
		for every component $o_i\notin\adom(J)\cup \vec v$, 
		$g(o_i)\notin\adom(I)\cup \vec u$.
		Thus, $g(\vec {o})\notin(\adom(I)\cup \vec u)^{\card{\vec x_1}}$.
		%%
		Now, because 
		$\vec o\in\varphi(\vec x_1,\vec v)^J\Ra J\models\varphi(\vec o, \vec v)$, 
		by Th.~\ref{prop:iso-eq}, 
		$I\models\varphi(g(\vec {o}),\vec u)$, 
		thus $g(\vec{o})\in \varphi(\vec x_1,\vec u)^I$.
		But $\varphi(\vec x_1,\vec u)^I$ is finite so, by Lemma~\ref{prop:fin-ans},
		$\varphi(\vec x_1,\vec u)^I\subseteq (\adom(I)\cup\vec u)^{\card{\vec x_1}}$.
		Contradiction.
		
		Since $\vec o\in(\adom(J)\cup \vec v)^{\card{\vec x_1}}$,
		$i^{-1}(\vec o)$ is defined. 
		Obviously, by definition of $\vec i$, \tup{\vec o,\vec v} is equivalent to 
		$i^{-1}(\tup{\vec o,\vec v})=\tup{i^{-1}(\vec o),\vec u}$.
		%%
		Thus, because $J\models\varphi(\vec o,\vec v)$,
		by Th.~\ref{prop:iso-eq},
		$I\models\varphi(i^{-1}(\vec o),\vec u)$, that is, 
		$i^{-1}(\vec o)\in\varphi(\vec x_1,\vec u)^I$.
	\end{comment}
\end{proofsk}

Thus, evaluating $\varphi(\vec x,\vec u)$ and $\varphi(\vec x,\vec v)$  
against A-isomorphic interpretations $I$ and $J$,
with equivalent input parameters $\vec u$ and $\vec v$, results,
for $\Delta^I$ infinite and $\Delta^J$ large enough,
in A-isomorphic answers 
(according to any A-isomorphism $i$ witnessing $I+\vec u\sim J+\vec v$).
%%
Importantly, $\Delta^J$ is not required to be infinite, a 
fact that we take advantage of in the next section.
%%

Finally, we define the notion of an
active-domain bisimulation relation, which essentially 
corresponds to standard bisimulation except for the 
fact that  the local condition requires bisimilar states 
to be  A-isomorphic. In details, given two labelled TSs
$T_1=\tup{\Delta_1,Q_1,q_{10},\ra_1,L_1}$ and 
$T_2=\tup{\Delta_2,Q_2,q_{20},\ra_2,L_2}$,
a relation $B\subseteq Q_1\times Q_2$ is an 
{\em active-domain bisimulation  relation} (\emph{A-bisimulation}, for short) between $T_1$ 
and  $T_2$ if $B(q_1,q_2)$ implies:
\begin{inparaenum}
	\item $L_1(q_1)\sim L_2(q_2)$;
	\item for every transition $q_1\ra_1 q_1'$, 
		there exists a transition $q_2\ra_2 q_2'$,
		s.t.~$\tup{q'_1,q'_2}\in B$;
	\item for every transition $q_2\ra_2 q_2'$, 
		there exists a transition $q_1\ra_1 q_1'$,
		s.t.~$\tup{q'_1,q'_2}\in B$.
\end{inparaenum}
%%
We say that $T_1$ and $T_2$ are {\em A-bisimilar}, written $T_1\approx
T_2$, if there exists an A-bisimulation relation $B$
s.t.~$\tup{q_{10},q_{20}}\in B$. As  usual, 
A-bisimilarity is an
equivalence relation.

Notice that  $T_1\approx T_2$ does not require
$\Delta_2$ to be infinite
(even if $\Delta_1$ is).
%%
Thus, there may and indeed does exist finite-state
TSs that are A-bisimilar to infinite-state ones.
%%
%%
%%For instance,  if every $q_1$ {\em reachable} from $q_{10}$ 
%%is s.t.~$\card{\adom(L_1(q_1))}\leq M$,
%%it is not hard to see that,
%%no matter how large $\Delta_1$ is,
%%there exists a bisimilar $T_2$ s.t.~$\card{\Delta_2}=M$.
%%
The central importance of this observation becomes apparent in light 
of Th.~\ref{mu-calc-iff} below, which states the invariance of $\mu\L$ wrt A-bisimulation.
%%
To introduce this result we need the notion of
domain-independent formulas.
We exploit our use of standard names to focus on sentences only.
%%
A sentence $\varphi\in\L_\D$ is said to be 
{\em domain-independent}~\cite{AbHV95} if 
for every interpretation
$I=\tup{\Delta^I,\cdot^I}$,
$I\models\varphi\Lra \hat I\models\varphi$,
where $\hat I=\tup{\adom(I),\cdot^I}$.
%%
Intuitively, domain-independent
sentences are those whose satisfaction 
depends only on $\cdot^I$.
%%
An example of domain-independent 
formula is 
$\exists x.Vehicle(x) \land \lnot Car(x)$,
and a domain-dependent variant
is $\exists x.\lnot Car(x)$.
%%
A $\mu\L$  formula is domain-independent
if so are all of its FO components 
(which are $\L_\D$ sentences).


%%
\begin{theorem}\label{mu-calc-iff}
	If $T_1\approx T_2$,
	then for every closed domain-independent $\mu\L$ formula $\varphi$,
	$T_1\models\varphi\Lra T_2\models\varphi$.
\end{theorem}
\begin{proofsk}
  The proof follows the standard proof of bisimulation-invariance of the
  $\mu$-calculus \cite{Stirling2001:Modal}, exploiting the fact that two states $q_1$
  and $q_2$ s.t.~$L(q_1)\sim L(q_2)$ satisfy the same domain-independent formulas.
\end{proofsk}

\begin{comment}
We close the section with a lemma, 
used in the next section,
which identifies sufficient conditions to guarantee that 
every tuple of elements from $\Delta^I$ has an equivalent 
counterpart from $\Delta^J$ and viceversa.
%%
\begin{lemma}\label{prop:iso-card}
	For every $n\geq 0$, if $I\sim J$, and 
	$\card{\Delta^I}=\card{\Delta^J}$ or
	$\card{\Delta^I},\card{\Delta^J}\geq N+n$, 
	%%where $N=\card{\adom(I)}=\card{\adom(J)}$,
	then for every $m\leq n$
	there exists $\vec o_I\in(\Delta^I)^m$
	iff 
	there exists $\vec o_J\in(\Delta^J)^m$
	s.t.~$\vec o_I$ and $\vec o_J$ are equivalent for $I$ and $J$.
\end{lemma}
%%
	\begin{proofsk}
		Let $i$ be an A-isomorphism from $I$ to $J$. 
		Given $\vec o_I\in(\Delta^I)^m$,
		it can be easily seen that,
		by the cardinality constraints on $\Delta^I$ and $\Delta^J$, 
		$i$ can be extended to $\vec o_I$, to a function $j$ 
		that is a bijection.
		%% 
		Thus, for $\vec o_J=j(\vec o_I)$, $\vec o_J$ is equivalent to $\vec o_I$.
		The opposite direction is proven analogously, by replacing $i$ with $i^{-1}$.
	\end{proofsk}
\end{comment}
%%



\subsection{Abstracting to Finite-State Transition Systems}
%%\textbf{FP: this should be moved to where transition systems are syntactically constructed.}
%%Observe that by applying the transformation of Th.~\ref{prop:sitcalc-fo-act}
%%and suppressing the situation term, we can reduce the evaluation 
%%of situation-calculus formulas, in particular action precondition and
%%successor state axioms, to that of FO-formulas. 
%%
%%So, given the current state, one can compute the 
%%state resulting from the application of an action without
%%taking the situation into account.
%%%%
%%It can be shown that by iteratively applying this step from 
%%the initial state, one can define a (situation-free) 
%%TS, whose states are those of $\M$,
%%that can be used  to verify the $\mu\L$ formulas 
%%of interest (whose atomic components are uniform, 
%%situation-suppressed sentences, that can thus be 
%%rewritten as FO-sentences).
%%%%
%%Unfortunately, even though this construction does not 
%%require the (infinite) model $\M$,
%%it is of no practical use, as the object sort,
%%and thus the states of the TS, is in general infinite.
%%%%
%%We prove later on that an equivalent
%%(from the verification point of view), finite (abstract) TS 
%%can be constructed as discussed above, but
%%using a finite object sort. This
%%construction cannot be carried out directly on 
%%$\M$, which is infinite even on finite object sorts, 
%%as containing the situation tree.
%%\textbf{FP}

%%
Next, we use the results devised so far to show how verification
against a bounded action theory can be reduced to that against a finite-state TS
whose states are interpretations of $\F$ over a finite abstract
domain.
%%


%%\textbf{GD: minor changes}
We first focus on domain-independent $\mu\L$ formulas.
By Th.~\ref{mu-calc-iff}, to check whether an infinite-state TS $T_1$ is s.t.~$T_1\models\varphi$,
we could try to construct an A-bisimilar finite-state $T_2$ 
and then check whether $T_2\models\varphi$.
%%
So, the question is whether such a $T_2$ actually exists.
%%
What we show next is that, 
under the boundedness assumption $T_2$ does exists and can be obtained 
by  essentially ``executing'' $\D$ over an 
interpretation domain of appropriate
finite cardinality.
%%

We start by giving counterpart of precondition and successor state axioms in $\L_\D$.
Recall that the form of such axioms is, respectively,
$\Poss(A(\vec x),s)\equiv \Pi_A(\vec x,s)$ and
$F(\vec x,do(a,s))\equiv\Phi_F(\vec x,a,s)$.
%%where 
%%$\Pi_A$ and $\Phi_F$ are situation-calculus formulas 
%%uniform in $s$,
%%s.t.~$\free(\Pi_A)\subseteq \vec x\cup\set{s}$ and
%%$\free(\Phi_F)\subseteq \vec x\cup\set{a,s}$.
%%
Observe that, by the unique name axioms for actions and domain closure for action types, 
the latter can be equivalently rewritten as 
$\bigwedge_{A\in\A} (F(\vec x,do(A(\vec y),s))\equiv\Phi_{FA}(\vec x,\vec y,s))$,
where $\vec y\notin\vars(\Phi_F)$ and each $\Phi_{FA}$ is obtained by 
syntactical substitution of $a$ by $A(\vec y)$ in $\Phi_F$. 
%%
Intuitively, this corresponds to having an instantiated successor
state axiom $F(\vec x,do(A(\vec y),s))\equiv\Phi_{FA}(\vec x,\vec y,s)$ per
action type.
%%
Then, for every righthand side of precondition axiom $\Pi_A$ and
instantiated successor state axiom $\Phi_{FA}$, we obtain equivalent
$\L_D$ formulas $\Pi'_A(\vec x)$ and $\Phi'_{FA}(\vec x,\vec y)$ via
Th.~\ref{prop:sitcalc-fo-act} and suppression of the situation
argument.
%%


Next, we observe that bounded action theories  
induce TSs with bounded state-labelings, that is,
for which there exists a bound $\beta$ 
s.t., for every state $q$ reachable from $q_0$ 
(i.e., every executable $\D$-situation),
$\card{\adom(L(q))}\leq \beta$.
%%
Intuitively, $\beta$ is the counterpart of the situation bound $b$
on the induced TSs.
%%
In the rest of the paper, 
given $b$, we assume
$\B=\sum_{F\in\F} b\cdot a_F$, 
with $a_F$ the arity of (the situation suppressed) $F$.
%%
This
is indeed a valid bound
for every TS induced by a $b$-bounded $\D$.
%%
%%
Also we denote by $\eta_p$ the maximum number of distinct variables occurring in the righthand side of the  action precondition and successor state axioms, once transformed into $\L_D$ as above:
$\eta_p= \max (\eta_{poss}\cup \eta_{ssa})$, 
where
%%\begin{inparaenum}
	%%\item 
$\eta_{poss}=\bigcup_{A(\vec x)\in\A}\set{\card{\vars(\Pi'_A(\vec x))}}$, and 
	%%\item 
$\eta_{ssa}=\bigcup_{F\in\F, A(\vec y)\in\A}
		\set{\card{\vars(\Phi'_{FA}(\vec x, \vec y))}}$.
%%\end{inparaenum}

                With these notions at hand, we can provide a
                sufficient condition to replace an infinite object
                domain with a finite one, while guaranteeing
                A-bisimilarity of the TSs induced by models of $\D$
                with such object domains.
%%
\begin{theorem}\label{th:ind-ts-bis}
  Given two TSs $T_1$ and $T_2$ induced by two models $\M_{\Delta_1}$ and $\M_{\Delta_2}$ with object domain
  $\Delta_1$ and $\Delta_2$, respectively, of a $b$-bounded action
  theory $\D$ (with initial situation described as a database), if $\Delta_1$ is infinite
  and $\card{\Delta_2}\geq \beta+\card{C}+\eta_p$, then $T_1\approx T_2$.
\end{theorem}
\begin{proofsk}
	The proof consists of proving that the relation 
	$B\subseteq Q_1\times Q_2$, s.t.~$B(q_1,q_2)$ 
	iff $L_1(q_1)\sim L_2(q_2)$, is a bisimulation relation.
	This requires the use of Th.~\ref{prop:sitcalc-fo-act}--\ref{prop:iso-query}, 
	to exploit the fact that every step 
%%	, \ref{prop:sitcalc-fo}, 
%%	\ref{prop:iso-eq}, Lemma~\ref{prop:iso-card}, and prop.~
	of the action theory depends only on the state, 
	and not on the situation.
	%%
	The cardinality requirement is needed to guarantee 
	that $\Delta_2$ is large enough to allow for the existence, 
	in $T_2$, of an A-isomorphic counterpart of each $T_1$-state.
	%%	
	\begin{comment}
		We prove that the relation 
		$B\subseteq Q_1\times Q_2$, s.t.~$B(q_1,q_2)$ 
		iff $L_1(q_1)\sim L_2(q_2)$, is a bisimulation relation.
		
		Observe that, by definition of induced TS, 
		$q_{10}=q_{20}$, thus  
		$L_1(q_{10})\sim L_2(q_{20})$ (in fact, all fluents 
		have exactly the same extension, in $L_1$ and $L_2$).
		
		Next assume $B(q_1,q_2)$. By definition of $B$,
		$L_1(q_1)\sim L_2(q_2)$.
		Consider a transition 
		$q_1\ra_1 q'_1$, and let $\M_1$ and $\M_2$ be the models 
		of $\D$ over $\Delta_1$ and $\Delta_2$, respectively.
		%%
		
		By definition of induced TS, 
		$q_1'=do(A(\vec o_1),q_1)$ and $\M_1\models \Poss(A(\vec o_1),q_1)$, 
		for some $A(\vec x)\in\A$, and $\vec o_1\in\Delta_1^{\card{\vec x}}$.
		%%
		Because $\Poss(A(\vec x),s)=\Pi_A(\vec x,s)$, 
		and $\Pi_A(\vec x,s)$ is uniform in $s$ 
		and without functional fluents, by 
		Th.~\ref{prop:sitcalc-fo-act},
		there exists a formula 
		$\Pi'_{A}(\vec x,s)$, where no action term occurs, 
		s.t.~$\M_1\models \Pi_A(\vec o_1,s)\Lra
		\M_1\models \Pi'_A(\vec o_1,s)$.
		%%
		But then, by 
		Th.~\ref{prop:sitcalc-fo},
		$\M_1\models \Pi'_A(\vec o_1,q_1)\Lra 
		L_1(q_1)\models \Pi'_A(\vec o_1)$,
		for $\Pi'_A(\vec x)$ obtained from $\Pi'_A(\vec x,s)$ by 
		suppressing $s$.
		%%
		Observe that
		$b\geq\card{\adom(L_1(q_1))}$, and, by $\eta_p$'s definition,
		$\eta_p\geq\card{\vars(\Pi'_A(\vec x))}$.
		%%
		Thus, 
		$\card{\Delta_2}\geq b+\card{C}+\eta_p\geq
		\card{\adom(L_1(q_1))}+\card{\vars(\Pi'_A(\vec x))}$.
		%%
		Since $L_1(q_1)\sim L_2(q_2)$ and 
		$\card{\vec x}\leq\card{\vars(\Pi'_A(\vec x))}$,
		by Th.~\ref{prop:iso-eq} and Lemma~\ref{prop:iso-card}, there exists
		$\vec o_2\in\Delta_2^{\card{\vec x}}$ equivalent to $\vec o_1$
		s.t.~$L_2(q_2)\models \Pi'_A(\vec o_2)$.
		%%
		Thus, by Th.~\ref{prop:sitcalc-fo},
		$\M_2\models \Pi'_A((\vec o_2),q_2)$.
		%%
		But then, observing  that $\Pi'_A(\vec x,s)$ is obtained from 
		$\Pi_A(\vec x,s)$ as shown in Th.~\ref{prop:sitcalc-fo-act},
		$\M_2\models \Pi_A((\vec o_2),q_2)$.
		%%
		Therefore, $\M_2\models \Poss(A(\vec o_2),q_2)$, and, 
		by definition of induced TS, 
		$q_2\ra_2 q'_2$, for $q'_2=do(A(\vec o_2),q_2)$.
		
		Now we prove that $L_1(q'_1)\sim L_2(q'_2)$.
		%%
		To this end, consider a generic successor state axiom
		$F(\vec x,do(a,s))=\Phi_F(\vec x,a,s)$, and observe that 
		$\Phi_F(\vec x,a,s)$ is 
		uniform in $s$ and contains no functional fluent. 
		Thus, for $A$ as above, by Th.~\ref{prop:sitcalc-fo-act}, 
		there exists a formula $\Phi_{FA}(\vec x,\vec y,s)$ uniform in $s$,
		containing no action term,
		and s.t.~$\const(\Phi_{FA})\subseteq\const(\Phi_F)\subseteq C$, 
		and
		$\M_1\models \Phi_F(\vec x,A(y),s)\Lra \M_1\models \Phi_{FA}(\vec x,\vec y,s)$,
		for every $\vec x$, $\vec y$, and $s$.
		Moreover, by Th.~\ref{prop:sitcalc-fo},
		$\M_1\models \Phi_{FA}(\vec x,\vec y,s) \Lra L_1(s)\models \Phi_{FA}(\vec x,\vec y)$,
		for $\Phi_{FA}(\vec x,\vec y)$ obtained by suppressing $s$ in $\Phi_{FA}(\vec x,\vec y,s)$.
		%%
		Thus, in particular for $q_1$ and $\vec o_1$ as above, 
		$\M_1\models \Phi_F(\vec x,A(\vec o_1),q_1)\Lra L_1(q_1)\models \Phi_{FA}(\vec x,\vec o_1)$, 
		and, by an analogous argument,  for $q_2$ and $\vec o_2$,
		$\M_2\models \Phi_F(\vec x,A(\vec o_2),q_2)\Lra L_2(q_2)\models \Phi_{FA}(\vec x,\vec o_2)$.
		
		
		Let
		$I'_1=L_1(q'_1)$ and $I'_2=L_2(q'_2)$. 
		%%
		By definition of induced TS,
		for every $F\in\F$, 
		$F^{I'_1}=\set{\vec o\mid \M_1\models F(\vec o,q'_1)}$ and
		$F^{I'_2}=\set{\vec o\mid \M_2\models F(\vec o,q'_2)}$.
		%%
		Observe that, since $T_1$ is $b$-bounded, 
		so is every $F^{I'_1}$ and $F^{I'_2}$.
		%%
		Moreover, because $F(\vec x,do(a,s))=\Phi_F(\vec x,a,s)$, 
		by the above results,
		$F^{I'_1}=\set{\vec o\mid L_1(q_1)\models \Phi_{FA}(\vec o,\vec o_1)}$, and 
		$F^{I'_2}=\set{\vec o\mid L_2(q_2)\models \Phi_{FA}(\vec o,\vec o_2)}$.
		%%
		Now, it can be seen that 
		$\card{\Delta_2}\geq b+\card{C}+\eta_p\geq
		\card{\adom(L_1(q_1))}+\card{\vars(\Phi_{FA}(\vec x,\vec y))}$.
		%%
		So, by Th.~\ref{prop:iso-query}, every witness 
		$i:\adom(L_1(q_1))\cup\vec o_1\mapsto\adom(L_2(q_2))\cup\vec o_2$
		of $I_1+ \vec o_1\sim I_2+\vec o_2$,
		where $I_1=L_1(q_1)$ and $I_2=L_2(q_2)$,
		is s.t., for every $F$, 
		$\vec o\in \Phi_{FA}(\vec x,\vec o_1)^{I_1}$ iff
		$i(\vec o)\in \Phi_{FA}(\vec x,\vec o_2)^{I_2}$.
		That is, for every $F$, 
		$\vec o\in F^{I'_1}$ iff $i(\vec o)\in F^{I'_2}$.
		%%
		But then, it is not hard to see that 
		$i|_{\adom(I'_1)}$ 
		is an A-isomorphism from 
		$I'_1$ to $I'_2$.
		%%
		Thus, $L_1(q'_1)\sim L_2(q'_2)$.
		
		Finally, consider a transition $q_2\ra_2 q'_2$.
		By the same argument as above, it can be proven that
		if $q'_2=do(A(\vec o_2),q_2)$, for some $A(\vec x)\in\A$
		and $\vec o_2\in\Delta_2^{\card{\vec x}}$,
		there exists an $\vec o_1\in\Delta_1^{\card{\vec x}}$ equivalent 
		to $\vec o_2$ s.t.~$q'_1=do(A(\vec o_1),q'_1)$, thus $q_1\ra_1 q'_1$.
		%%
		Once $\vec o_1$ is defined, 
		the fact that $L_1(q'_1)\sim L_2(q'_2)$, 
		can be proven in the same way as above.
	\end{comment}
\end{proofsk}
%%
%%Observe that although, by $\Delta_2$'s finiteness, 
%%only finitely many possible labelings exist 
%%in $T_2$,  $Q_2$ is still infinite. 
%%Thus, it cannot be neither constructed nor inspected 
%%to check whether it satisfies a given formula.
%%

Finally, we show that we can avoid the construction of the induced TS
$T_2$ of the above theorem, which is infinite though over a
finite object domain, by resorting to a direct construction of a TS $\hat{T}$ that
is A-bisimilar to $T_2$.
%%
Intuitively, this is done by executing $\D$,
from $\D_0$,
on a finite $\hat\Delta$ that satisfies the 
requirements of Th.~\ref{th:ind-ts-bis}. 
%%
The construction is %technically
made possible by
Th.~\ref{prop:iso-query}, which essentially 
states that
executing an action type with equivalent tuples 
from A-isomorphic states
leads to A-isomorphic successor states.
%%
Formally, for a $b$-bounded action theory $\D$, we define a {\em
  bounded abstract TS} of $\D$ as a TS $\hat T=\tup{\hat\Delta,\hat
  Q,\hat q_0,\hat \ra,\hat L}$, s.t.:
\begin{inparaenum}
	\item $C\subseteq \hat\Delta$ and $\card{\hat \Delta}=\beta+\card{C}+\eta_p$;
	\item $\hat Q\subseteq Int^\F_{\hat\Delta}$;
	\item for every $F\in\F$, $\vec o\in F^{\hat q_0}$ iff $\D_0\models F(\vec o)$;
	\item $\hat q\hat\ra\hat q'$ iff:
		\begin{inparaenum}
			\item there exists $A(\vec y)\in\A$ s.t., 
				for some $\vec o_A\in\hat\Delta^{\card{\vec y}}$, 
				$\hat q\models \Pi'_A(\vec o_A)$;
			\item for every $F\in\F$, $\vec o\in F^{\hat q'}$ iff $\hat q\models \Phi'_{FA}(\vec o, \vec o_A)$;
%%				for $\Phi'_{FA}(\vec x,\vec y)$ is obtained from the successor state axiom 
%%				$\Phi_F(\vec x,a,s)$, for the action type $A$, as shown above;
		\end{inparaenum}
	\item $\hat L$ is the identity.
\end{inparaenum}
%%
%%Obviously, given $\hat\Delta$, $\hat T$
%%can be actually constructed, as $\hat \Delta$ is
%%finite. 
%%
%%We can now show that $\hat T$ is A-bisimilar to
%%the transition system $T_2$ induced by $\D$ over 
%%$\hat\Delta$. 
%%To this end, we introduce first the following intermediate result.
%%
%%
% \begin{proposition}\label{prop:discard-sit}
% {\bf FP: no longer sure this proposition is useful. It is never used.}
%{\bf GDG: embedded in the proof of Proposition~\ref{prop:sitcalc-fo}}
% Given an action theory $\D$, 
% for every two situations $s$ and $s'$ of the
% model $\M$ of $\D$ over $\Delta$, 
% if, 
% for every $F\in\F$, 
% $\set{\vec o\mid \M\models F(\vec o, s)}=
% \set{\vec o\mid \M\models F(\vec o, s')}$
% then:
% 	\begin{inparaenum}
% 		\item for every $A(\vec x)\in\A$,
% 			$\M\models\Poss(A(\vec x),s)\Lra
% 			\M\models\Poss(A(\vec x),s')$;
%
% 		\item	for every $F\in\F$,
% 			$\M\models F(\vec x,do(a,s))\Lra
% 			\M\models F(\vec x,do(a,s'))$.
% 	\end{inparaenum}
% \end{proposition}
% %%
% \begin{proofsk}
%  	The thesis follows  
% 	by prop.~\ref{prop:sitcalc-fo}, 
% 	which applies because action 
% 	precondition axioms 
% 	and successor state axioms 
% 	contain no functional fluents and 
% 	are uniform in the 
% 	situation argument, thus they depend only
% 	on the state.
% \end{proofsk}
% %%

Then, we can state our abstraction result.
%%
\begin{theorem}\label{th:abs-exec}
  Let $\hat T$ be a  bounded abstract TS of $\D$ with object
  domain $\hat\Delta$, and $T_2$ be the TS induced by a model $\M_{\hat \Delta}$ of $\D$
  with object domain $\hat\Delta$. Then, $T_2\approx \hat T$.
\end{theorem}
%%
\begin{proofsk}
		We  prove that the 
		relation $B\subseteq \hat Q\times Q_2$
		s.t.~$B(\hat q,q_2)$ iff $\hat q=L_2(q_2)$ is an 
		A-bisimulation s.t.~$B(\hat q_0,q_{20})$, where $q_{20}$ 
		is the initial state of $T_2$.
	\begin{comment}
		Let $\M_2$ be the model of $\D$ over $\hat\Delta$, and
		consider the definition of $\hat T$.
		The proof consists of proving that the 
		relation $B\subseteq \hat Q\times Q_2$
		s.t.~$B(\hat q,q_2)$ iff $\hat q=L_2(q_2)$ is a 
		bisimulation relation s.t.~$B(\hat q_0,q_{20})$.
		
		The fact that $B(\hat q_0,q_{20})$ is obvious.
		%%
		To see that $B$ is a bisimulation relation, consider a 
		pair $\tup{\hat q,q_2}\in B$. 
		Obviously, because $\hat L$ is the identity, 
		$\hat L(\hat q)=\hat q=L_2(q_2)$, thus $\hat L(\hat q)\sim L_2(q_2)$.
		
		Next, assume that $q_2\ra_2 q'_2$. 
		By definition of induced TS, 
		there exists an action $A(\vec o_A)$ 
		s.t.~$\M_2\models\Poss(A(\vec o_A),q_2)$, and 
		$q'_2=do(A(\vec o_A),q_2)$.
		%%
		For $\Poss(A(\vec x),s)=\Pi_A(\vec x,s)$, 
		by  Th.~\ref{prop:sitcalc-fo-act} 
		and~\ref{prop:sitcalc-fo}, and definition of induced
		TS, 
		$\M_2\models\Poss(A(\vec o_A),q_2)$ iff
		$L_2(q_2)\models \Pi'_A(\vec o_A)$. Thus, 
		being  $\hat q=L_2(q_2)$,
		$\hat q\models \Pi'_A(\vec o_A)$. 
		%%
		Similarly, we can prove that, 
		for every $F\in\F$, 
		$\M_2\models F(\vec o,do(A(\vec o_A),q_2))\Lra
		L_2(q_2)\models \Phi_{FA}(\vec o,\vec o_A)$.
		That is, by definition of induced TS, and being 
		$q'_2=do(A(\vec o_A),q_2)$,
		$L_2(q'_2)\models F(\vec o)\Lra 
		L_2(q_2)\models \Phi_{FA}(\vec o,\vec o_A)$.
		Thus, for $\hat q'=L_2(q'_2)$,
		because $\hat q=L_2(q_2)$, 
		$\hat q'\models F(\vec o)$ iff 
		$\hat q\models \Phi_{FA}(\vec o,\vec o_A)$.
		But then, by the way $\hat T$ is defined,
		$\hat q\hat\ra\hat q'$. 
		$B(\hat q', q'_2)$ 
		is an immediate consequence of 
		$\hat q'=L_2(q'_2)$.
		
		The other direction is proven similarly.
		Assuming that $\hat q\hat\ra \hat q'$,
		by definition of abstract TS, for some 
		$\vec o_A$, $\hat q\models\Pi'_A(\vec o_A)$.
		Being $\hat q=L_2(q_2)$, this holds iff
		$L_2(q_2)\models\Pi'_A(\vec o_A)$, that is, 
		by  Th.~\ref{prop:sitcalc-fo-act} 
		and~\ref{prop:sitcalc-fo}, iff 
		$\M_2\models\Poss(A(\vec o_A),q_2)$.
		Thus, for $q'_2=do(A(\vec o_A),q_2)$, 
		by definition of induced TS, $q_2\ra_2 q'_2$.
		%%
		To see that $B(\hat q',q'_2)$, observe that,
		as shown above, for every $F\in\F$, 
		$\M_2\models F(\vec o,q'_2)\Lra
		L_2(q_2)\models \Phi_{FA}(\vec o,\vec o_A)$, and, 
		by definition of induced TS,
		$L_2(q'_2)\models F(\vec o)\Lra \M_2\models F(\vec o,q'_2)$.
		Therefore, 
		$L_2(q'_2)\models F(\vec o)\Lra L_2(q_2)\models \Phi_{FA}(\vec o,\vec o_A)$.
		%%
		Moreover, by definition of abstract TS, for every $F\in\F$, 
		$\hat q'\models F(\vec o)\Lra 
		\hat q\models \Phi_{FA}(\vec o, \vec o_A)$.
		But then, because $\hat q=L_2(q_2)$,
		for every $F\in\F$, 
		$\hat q'\models F(\vec o)\Lra 
		L_2(q_2)\models \Phi_{FA}(\vec o, \vec o_A)$.
		Thus, it can be seen that $\hat q'=L_2(q'_2)$, 
		therefore $B(\hat q',q'_2)$.
	\end{comment}
\end{proofsk}

Since by Th.~\ref{th:ind-ts-bis}, $T_2\approx T_1$, 
for $T_1$ the transition system induced by \emph{the} model $\M$ of $\D$ (with object domain $\N$),
we have $\hat T\approx T_2\approx T_1$, thus, $\hat T\approx T_1$.
Therefore, by Th.~\ref{mu-calc-iff} and Th.~\ref{th:InducedTS}, we have the following result.
%%
\begin{theorem}\label{th:abs-th}
  Given a $b$-bounded action theory $\D$ (with initial situation
  described as a database) and a $\mu\L$ closed, domain-independent
  formula $\Phi$, let $\hat T$ be a bounded abstract TS of $\D$. Then,
  $\D\models\Phi\Lra\hat T\models\Phi.$
\end{theorem}
%%
Therefore, verifying a $b$-bounded action theory against a $\mu\L$ closed formula
$\Phi$ that is domain-independent is decidable, as $\hat T$ 
is finite, thus can be actually constructed, and checking whether 
$\hat T\models\Phi$ is decidable.

% To conclude the proof of Th.~\ref{th:dec-verif}, we need to extend this result
% to general $\mu\L$ formulas.

\subsection{Relaxing the Domain-Independence Assumption}
%%Since a bounded abstract $\hat T$ 
%%can be actually constructed, 
%%as $M$ and $\eta_p$ can be derived 
%%from a $b$-bounded $\D$, 
%%Th.~\ref{th:abs-th}
%%states that the verification of 
%%bounded action theories is decidable 
%%for {\em domain-independent} 
%%$\mu\L$ formulas. 
%%
To conclude the proof of Th.~\ref{th:dec-verif}, we need to extend 
Th.~\ref{th:abs-th} to general $\mu\L$ formulas.
%Finally, we generalize Th.~\ref{th:abs-th}
%to full $\mu\L$, thus obtaining a proof of Th.~\ref{th:dec-verif}.
%%
This is easily done by adapting to our 
framework a classical result, see e.g.,~\cite{Libkin07}, that essentially 
defines a syntactic transformation to make arbitrary FO formulas
domain-independent.
%%
\begin{theorem}\label{th:libkin}
  For every $\L_\D$ formula $\varphi$ there exists a
  domain-independent $\L_\D$ formula $\varphi'$ such that $\forall
  (\varphi \equiv \varphi')$.
 %        There exists a polynomial transformation 
 %        that, given an arbitrary $\L_\D$ formula $\varphi$,
 %        generates a domain-independent $\L_\D$  formula $\varphi'$ such that 
 % $\forall (\varphi \equiv \varphi')$.
\end{theorem}
%%
\newcommand{\ADOM}{\texttt{adom}}
\begin{proofsk}
Let $\ADOM$ be a FO formula
s.t.~for every interpretation $I$ and object $o\in\N$, 
$I\models \ADOM(o)$ iff $o\in\adom(I)$. 
Such a formula can be proven to exist.
%%
Define the syntactic transform 
$\tau$ of an FO formula $\phi$ by induction, as follows:
if $\phi$ is atomic,  
$\phi=\lnot \phi'$, 
or $\phi=\phi'\land\phi''$,
then, respectively,
$\tau(\phi)=\phi,~\lnot\tau(\phi'),~\tau(\phi')\land\tau(\phi'')$;
%%
else, assuming w.l.o.g.~$\phi=\exists x.\psi(x,\vec z)$,
%%
% $\tau(\phi)=
% \big(
% 	\exists x.\ADOM(x)
% 	\land
% 	\big(
% 		(\exists y. \ADOM(y)\wedge(\tau(\psi[x/y])))
% 		\vee 
% 		(\bigvee_{i=1}^{\card{\vec z}}(\tau(\psi[x/z_i])))
% 		\vee
% 		(\tau(\psi[x/w]))
% 	\big)
% \big)
% \vee 
% (\lnot\exists x.\ADOM(x)\land \tau(\phi_\emptyset))$,
\[\begin{array}{l}
\tau(\phi)= \exists y.\ADOM(y) \land{}
			\big( \exists x.\ADOM(x) \land  \tau(\psi(x,\vec z))
				\vee \\
				\bigvee_{i=1}^{\card{\vec z}}\tau(\psi(z_i,\vec z))
				\vee 
				\tau(\psi(w,\vec z))
			\big)\lor
			\lnot 
			\exists y.\ADOM(y) \land \tau(\phi_\emptyset)
\end{array}
\]
where: \myi $w$ is a fresh variable symbol not occurring in $\phi$, and \myii
$\phi_\emptyset$ is 
%%a quantifier-free formula equivalent to that 
obtained from $\phi$ by replacing 
each subformula of the form $F(\vec t)$ with $\false$.
%%
Let $\varphi_\tau=\tau(\varphi)$, and
$W$ be the set of all variables of 
type $w$ introduced by $\tau$,
when generating $\varphi_\tau$.
%%
Finally, obtain $\varphi'$ 
from $\varphi_\tau$ by
replacing: 
each subformula $w=w$  with $\true$,  and each subformula  $w=y$ where $y$ is a variable symbol different from
$w$, and $F(\ldots,w,\ldots)$  with $\false$.
%%
It is easy to show that
$\varphi'$ is domain-independent and 
equivalent to $\varphi$.
\end{proofsk}
%%
Thus, by applying the syntactic transformation in the proof of the above
theorem to each FO component of a $\mu\L$ formula $\Phi$,
Th.~\ref{th:abs-th} generalizes immediately to Th.~\ref{th:dec-verif}.







%%% Local Variables:
%%% mode: latex
%%% dirvars: nil
%%% save-place: t
%%% TeX-master: "main"
%%% End:



==> 52-mu-calc-ts.tex <==
\subsection{$\mymu$ over Transition Systems}
\label{sec:mu-calc-ts}

The results presented in Section~\ref{sec:action-suppression} and
\ref{sec:situation-suppression} suggest that, for the purpose of
verification of $\mymu$ formulas, one can operate on simpler structures
 than the models of situation calculus action theories. Indeed, as it turns out,
both actions and situations can be somehow disregarded.
%%
In this section, we introduce such simpler structures, namely
\emph{transition systems} (TS),
show  how $\mymu$ formulas are evaluated over them, and 
present some important results.
%%
The connection between models of situation calculus theories 
and transition systems will be discussed in Section~\ref{sec:ind-ts}.
%%
By Theorem~\ref{prop:sitcalc-fo-act}, we can focus, without loss of generality,
on a variant of $\mymu$
%%
%%Notice that in $\mymu$ there cannot be occurrences of situation terms,
%%since all FO formulas are uniform situation-suppressed situation
%%calculus formulas. As a result, the only predicates that occur in
%%$\mymu$ formulas are fluents or equalities between terms,
%%including action terms. However, considering that there are
%%only finitely many action types and that we unique name assumption 
%%and domain closure on actions, we can rephrase all equalities between 
%%action terms into equalities on object terms. 
%%So, without loss of generality, 
where action terms are disallowed.

By $Int^{\F,C}_\Delta$, we denote the set of all possible interpretations of the situation suppressed fluents 
in $\F$ and  constants in $C$ (e.g.\ the one occurring ina an action theory $\D$), over an object domain $\Delta$.
%%
A {\em transition system} (TS) (over the situation-suppressed fluents
$\F$, constants $C$, and object domain $\Delta$) is a tuple
$T=\tup{\Delta,Q,q_0,\ra,\I}$, where:
%\begin{inparaenum}
\begin{itemize}\itemsep=0pt
	\item $\Delta$ is the {\em object domain};
	\item $Q$ is the {\em set of states};
	\item $q_0\in Q$ is the {\em initial state};
	\item $\ra\subseteq Q\times Q$ is the {\em transition relation}; and
	\item $\I:Q\mapsto Int^{\F,C}_\Delta$ is the {\em labeling function} associating each state $q$ with an 
	interpretation $\I(q)=\tup{\Delta,\cdot^{\I(q)}}$ such that the constants in $C$ are 
	interpreted in the same way in all the states over which $\I$ is defined.
\end{itemize}
%\end{inparaenum}

To interpret a $\mymu$ formula over a TS $T=\tup{\Delta,Q,q_0,\ra,\I}$, 
we use valuation $(\vfo, \vso)$ formed by an individual variable valuation $\vfo$ and a parametrized predicate variable
valuation $\vso$, as in Section~\ref{sec:mucalc}. To express that $\vfo$ assigns the values $\vec d$ to 
the variables $\vec x$, we use the notation $\vec x/\vec d\in\vfo$.
Further, for an individual variable valuation $\vfo$, by 
$\vfo[\vec x/\vec d]$ we mean the valuation $\vfo'$ analogous to $v$ except 
for the fact that $\vec x/\vec d\in\vfo'$. Finally, for an interpretation $\I$, 
we write $\vec d\subseteq\adom(\I)$ to express that all the individuals occurring 
in $\vec v$ (as components) come from $\adom(\I)$. Similarly, we write 
$\vec d\subseteq S$ for a generic set $S$.
We can now define the \emph{extension function}
\label{def:modat}
$\MODAT{\cdot}$, which maps $\mymu$ formulas to subsets of $Q$, as follows:
\[\begin{array}{lcl}
\MODAT{\varphi} &= & \{q \in Q\mid \I(q),v\models \varphi \}\\
\MODAT{\lnot \Phi} &= & Q - \MODAT{\Phi} \\
\MODAT{\Phi_1 \land \Phi_2} &= &\MODAT{\Phi_1}\cap\MODAT{\Phi_2}\\
\MODAT{\exists x.\,\inadom(x)\land\Phi} &=&
      \{q \in Q\mid\exists d\in \adom(\I(q)).\, q \in \MODATX{\Phi}{[x/d]}\}\\
\MODAT{\inadom(\vec{x})\land \DIAM{\Phi}} &=&
      \{q\in  Q\mid \vec{x}/\vec{d} \in \vfo \mbox{ and } \vec{d}\subseteq\adom(\I(q)) \mbox{ and }\\
      & & \quad\exists q'.  q\ra q'\mbox{ and } q' \in \MODAT{\Phi}\} \\
\MODAT{\inadom(\vec{x})\land \BOX{\Phi}} &=&
      \{q\in Q \mid \vec{x}/\vec{d} \in \vfo \mbox{ and } \vec{d}\subseteq\adom(\I(q)) \mbox{ and }\\
    & & \quad\forall q' .\, q \ra q' \mbox{ implies } q'\in \MODAT{\Phi}\} \\
\MODAT{Z} &= & \vso(Z)\\
\MODAT{\mu Z.\Phi} &= & \bigcap\{\E\subseteq Q \mid \MODATZ{\Phi}{[Z/\E]}
\subseteq \E \}%\\
\end{array}
\]

Given a $\mymu$ formula $\Phi$, we say that a transition system $T$ \emph{satisfies
$\Phi$ at state $q$, under $v$ and $V$}, written $T,q,(\vfo,\vso)\models\Phi$, if 
$q\in \MODAT{\Phi}$. When $\Phi$ is closed on predicate variables, 
we omit $\vso$ as not relevant and write simply $T,q\models\Phi$. If $\Phi$ is closed on both individual and predicate variables we write $T,q,\vfo\models\Phi$. For closed formulas,
we say that \emph{$T$ satisfies $\Phi$}, written $T\models\Phi$, if $T,q_0\models\Phi$.

For our TSs we can restate the classical \emph{bisimulation invariance
results} for the $\mu$-calculus, which state that bisimilar TSs satisfy
exactly the same $\mu$-calculus formulas --see,
e.g.,~\cite{BS07}. Hence we have that all the
TSs that are bisimilar to the one induced by a situation calculus
model (cf.\ Sect.~\ref{sec:ind-ts}), satisfy exactly the same formulas, even if their transition
relation does not reflect the tree structure induced by the situation
tree.  Obviously, the notion of bisimulation needed here is not the
classical one, but one that takes into account the FO interpretations
labeling the states of the transition systems, as well as the
controlled form of quantification across states allowed in $\mymu$.

%%FP: partial bijections not needed anymore

\begin{comment}
In order to formally define the notion of bisimulation used in this paper, 
we first fix some terminology.
A \emph{partial bijection} $h$ between two (object) domains $\Delta_1$
and $\Delta_2$ is a bijection between a subset of $\Delta_1$ and
$\Delta_2$. Given a set $D\subseteq \Delta_1$, $\restrict{f}{D}$ denotes
the \emph{restriction} of $f$ to $D$, i.e., the function such that
$\domain{\restrict{f}{D}} = \domain{f} \cap D$
and $\restrict{f}{D}(x) = f(x)$ for every $x \in \domain{f} \cap D$,
with $\domain{f}$ the set of objects over which $f$ is defined.
%
We say that a function $f'$ \emph{extends} a function $f$
if $\restrict{f'}{\domain{f}}(x)=f(x)$, for all $x\in\domain{f}$.
Let $\I_1$ and $\I_2$ be two FO interpretations (both over the situation
suppressed fluents of $\D$)
over domains $\Delta_1$ and $\Delta_2$, respectively, and let $C_1$ and $C_2$
be the set of their constants.
We say that a partial bijection $h$
\emph{induces an isomorphism} between $\I_1$ and $\I_2$ if
$\adom(\I_1)\cup C^{\I_1}\subseteq \domain{h}$, for 
$C^{\I_i}=\set{c^{\I_i}\mid c\in C_i}$ ($i=1,2$),
$\adom(\I_2)\cup C^{\I_2}\subseteq \image{h}$,
and $\restrict{h}{\adom(\I_1)\cup C^{\I_1}}$ is an isomorphism between 
$\tup{\adom(\I_1)\cup C^{\I_1},\cdot^{\I_1}}$ and $\tup{\adom(\I_2)\cup C^{\I_2},\cdot^{\I_2}}$.
%%%%
Observe that in order for a partial bijection to exist from $\Delta_1$ to $\Delta_2$, 
it must be the case that $\card{\Delta_1}\geq \card{\Delta_2}$.
\end{comment}


We first recall the standard 
notions of \emph{isomorphism} and \emph{isomorphic interpretations}. 
Two FO interpretations
$\I_1=\tup{\Delta_1,\cdot^{\I_1}}$ and $\I_2=\tup{\Delta_2,\cdot^{\I_2}}$,
over the same fluents $\F$ and constants $C$,
are said to be \emph{isomorphic}, written $\I\sim\I'$,
if there exists a bijection (called \emph{isomorphism}) 
$\iota:\Delta_1\mapsto\Delta_2$ such that:
\myi for every $F\in\F$, $\vec x\in F^{\I_1}$ if and only if $\iota(\vec x)\in F^{\I_2}$;
\myii for every $c\in C$, $c^{\I_2}=h(c^{\I_1})$. 
%%
Notice that, necessarily, the interpretation domains of isomorphic interpretations
have same cardinality.
%%
Intuitively, for two interpretations to be isomorphic, it is required that one 
can be obtained from the other by renaming the individuals in the interpretation 
domain.
%%
When needed, to make it explicit that $\iota$ is an isomorphism between $\I_1$ and
$\I_2$, we write $\I_1\sim_\iota \I_2$.
%%
It is immediate to see that if $\iota$ is an isomorphism, then so is $\iota^{-1}$, and that 
$\sim$ is an equivalence relation.
%%An equivalence class of isomorphic interpretations is
%%called an \emph{isomorphism type}.
%%

Given a function $f:D_1\mapsto D_2$ and a set $D'_1\subseteq D_1$,
let $f(D'_1)\subseteq D_2$ denote the \emph{image of $D'_1$ through $f$}, i.e., the 
set of elements $d_2\in D_2$ such that $d_2=f(d_1)$, for some $d_1\in D_1$.
We denote by $\restrict{f}{D'_1}$ the \emph{restriction} of $f$ to $D'_1$, i.e., the function
$\restrict{f}{D'_1}:D'_1\mapsto f(D'_1)$, such that $\restrict{f}{D'_1}(d)=f(d)$, for every $d\in D'_1$.
%%
Recall the definition of \emph{restriction of an interpretation} $\I=\tup{\Delta,\cdot^\I}$
to its active domain, i.e., $\arestrict{\I}=\tup{\adom(\I),\cdot^{\I}}$,
and consider two interpretations $\I_1=\tup{\Delta_1,\cdot^{\I_1}}$, 
$\I_2=\tup{\Delta_2,\cdot^{\I_2}}$, and a function 
$f:\Delta_1\mapsto\Delta_2$.
If $\restrict{f}{\adom(\I_1)}$ is such that 
$\arestrict{\I_1}\sim_{\restrict{f}{\adom(\I_1)}}\arestrict{\I_2}$, 
we write, for simplicity, $\arestrict{\I_1}\sim_f \arestrict{\I_2}$, even if $f$ itself is not 
an isomorphism. Intuitively, this means that $f$ induces a bijection between the active
domains of $\I_1$ and $\I_2$ that preserves the interpretation of fluents.
In fact, $f$ might not even be a bijection 
(while its restriction $\restrict{f}{\adom(\I_1)}$ must be).
%%
Notice that if, for some function $f:\Delta_1\mapsto\Delta_2$, it is the case that 
$\arestrict{\I_1}\sim_f \arestrict{\I_2}$, then any changes to
$f$ outside $\adom(\I_1)$ do not affect the property that 
$\arestrict{\I_1}\sim_{f} \arestrict{\I_2}$. In particular,
any arbitrary extension $f'$ of  $\restrict{f}{\adom(\I_1)}$ to a superset $D$ of $\adom(\I_1)$,
is such that $\arestrict{\I_1}\sim_{f'} \arestrict{\I_2}$. 
We use these facts in the following.

The bisimulation relation % --inspired by that in~\cite{BelardinelliLP14}--
that captures \mymu  can be defined as follows.  
%%
Let $T_1 = \tup{\Delta_1,Q_1,q_{10},\ra_1,\I_1}$ and
$T_2= \tup{\Delta_2, Q_2, q_{20}, \ra_2, \I_2}$ 
be two transition systems
(over the situation-suppressed fluents and constants of an action theory $\D$).
%%
A relation $B\subseteq \Delta_1\times \Delta_2$ is a
\emph{persistence-preserving bisimulation}\label{def:bisim}
between $T_1$ and $T_2$,
if $\tup{q_1,q_2}\in B$ implies that:
\begin{enumerate}
\item\label{bisim:req1} 
	$\arestrict{\I_1}(q_1)\sim_h\arestrict{\I_2}(q_2)$, for some function $h:\Delta_1\mapsto\Delta_2$;

\item\label{bisim:req2} for each $q_1'\in Q_1$, if $q_1 \ra_1 q_1'$ then there exist
  $q_2'\in Q_2$ such that $q_2 \ra_2 q_2'$ and a function 
  $h':\Delta_1\mapsto\Delta_2$ that extends $\restrict{h}{\adom(\I_1(q_1))}$, such that $\arestrict{\I_1}(q'_1)\sim_{h'}\arestrict{\I_2}(q'_2)$
  and  $\tup{q_1',q_2'}\in B$;
  
\item\label{bisim:req3} for each $q_2'\in Q_2$, if $q_2 \ra_2 q_2'$ then there exist 
$q_1'\in Q_1$ such that~$q_1 \ra_1 q_1'$ and a function 
$h':\Delta_1\mapsto\Delta_2$ that extends $\restrict{h}{\adom(\I_1(q_1))}$, such that $\arestrict{\I_1}(q'_1)\sim_{h'}\arestrict{\I_2}(q'_2)$
  and  $\tup{q_1',q_2'}\in B$.
\end{enumerate}
%%
%%%%FP: Old definition
%%%%Let $T_1 = \tup{\Delta_1, Q_1,q_{10},\ra_1, \I_1}$ and 
%%%%$T_2 =\tup{\Delta_2, Q_2,q_{20},\ra_2, \I_2}$ be two transition systems 
%%%%(over the situation-suppressed fluents and constants of an action theory $\D$),
%%%%and let $H$ be the set of all possible bijections between $\Delta_1$ and $\Delta_2$.
%%%%A \emph{persistence-preserving bisimulation}\label{def:bisim} between $T_1$ and $T_2$
%%%%is a relation $B \subseteq Q_1 \times H \times Q_2$ such that
%%%%$\tup{q_1,h,q_2} \in B$ implies:
%%%%\begin{enumerate}
%%%%\item\label{bisim:req1} $\I_1(q_1)\sim_h\I_2(q_2)$;
%%%%\item\label{bisim:req2} for each $q_1'$, if $q_1 \ra_1 q_1'$ then there exist
%%%%  $q_2'$ such that $q_2 \ra_2 q_2'$ and a bijection $h'$ that
%%%%  extends $\restrict{h}{\adom(\I_1(q_1))}$,
%%%%  such that $\tup{q_1',h',q_2'}\in B$;
%%%%\item\label{bisim:req3} for each $q_2'$, if $q_2 \ra_2 q_2'$ then there exist $q_1'$
%%%%  such that~$q_1 \ra_1 q_1'$ and a bijection $h'$ that extends
%%%%  $\restrict{h}{\adom(\I_1(q_1))}$, such that
%%%%  $\tup{q_1',h',q_2'}\in B$.
%%%%\end{enumerate}
Notice that the requirement on $h'$ at \ref{bisim:req2} (and \ref{bisim:req3}) 
essentially imposes that $h'$ preserves the mappings of $h$ on the objects
shared by $\I(q_1)$ and $\I(q'_1)$ (and $\I(q_2)$ and $\I(q'_2)$), that is, that 
their ``identity'' is preserved along the transition.

We say that a state $q_1 \in Q_1$ is \emph{persistence-preserving
 bisimilar} to $q_2 \in Q_2$,%% \emph{wrt a bijection} $h$,
written $q_1 \approx q_2$, if there exists a persistence-preserving
bisimulation $B$ between $T_1$ and $T_2$ such that
$\tup{q_1,q_2}\in B$.
%%We simply say that 
%%$q_1 \in Q_1$ is \emph{persistence-preserving bisimilar} to
%%$q_2 \in Q_2$, written $q_1 \approx q_2$, if $q_1 \approx_h q_2$,
%%for some $h$.
Finally, a transition system $T_1$ is said to be \emph{persistence-preserving
  bisimilar} to $T_2$, written $T_1 \approx T_2$, if
$q_{10} \approx q_{20}$. It is immediate to see that bisimilarity 
between states and transition systems, i.e., the (overloaded) relation $\approx$, 
is an equivalence relation.
%%

Next, we prove a result (Theorem~\ref{thm:mymu-bisimulation})
saying that \mymu enjoys invariance under this
notion of bisimulation. To this end, 
we first show the result for the simpler logic $\myhm$, obtained
from $\mymu$ by dropping the predicate variables and the fixpoint
constructs (see Lemma~\ref{lemma:myhm-bisimulation}). Such a logic corresponds to a first-order variant of the
Hennessy-Milner Logic \cite{HM80}; note that its semantics is
completely independent from the second-order valuation. 
%%

% \begin{lemma}\label{lemma:myhm-bisimulation}
%   Consider two transition systems $T_1= \tup{\Delta_1,Q_1,q_{10},\ra_1,\I_1}$
%   and $T_2= \tup{\Delta_2, Q_2, q_{20}, \ra_2, \I_2}$,
% 	both with infinite object domain,
%     and two states $q_1\in Q_1$, $q_2 \in Q_2$,
%   such that  $q_1 \approx q_2$ and $\arestrict{\I_1}(q_1) \sim_h \arestrict{\I_2}(q_2)$.
% %  
%    For every (open) formula $\Phi$ of $\myhm$ 
%   and every two valuations $\vfo_1$, $\vfo_2$ such that 
%   $\vfo_1(\vec x)= \vec d_1\in \vec\Delta_1$ and $\vfo_2(\vec x)= \vec d_2\in \vec\Delta_2$, 
%   	if $\vec d_2 = h(\vec d_1)$ or $\vec d_i\notin \vec \adom(\I_i(q_i))$ 
%   	($i=1,2$) then 
% \[T_1,q_1,\vfo_1 \models \Phi \, \textrm{ if and only if }\,  T_2,q_2,\vfo_2 \models \Phi . \]
% \end{lemma}
% \begin{proof}
%   We proceed by induction on the structure of $\Phi$, assuming that $x$ is the 
%   only free variable of $\Phi$, and that $\vfo_1(x)=d_1$. 
  
%   The cases of boolean connectives are straightforward.

%   For $\Phi=\varphi$, we observe that, by Theorem~\ref{thm:dom-ind}, 
%  $\I_i(q_i),\vfo_i\models\varphi$ if and only if $\arestrict{\I_i}(q_i),\vfo_i\models\varphi'$
%  ($i=1,2$),
%   for $\varphi'$ the rewriting of $\varphi$ as its domain-independent version.
%   Further, because $\arestrict{\I_1}(q_1)\sim_h\arestrict{\I_2}(q_2)$, 
%   by the invariance of  FOL wrt isomorphic interpretations, it follows that 
%   $\arestrict{\I_1}(q_1),\vfo_1\models\varphi'$ if and only if 
%   $\arestrict{\I_2}(q_2),\vfo_2\models\varphi'$ (either if $d_2 = h(d_1)$ or 
%   $d_i\notin \adom(\I_i(q_i))$). 
%   These two facts easily imply the thesis.
  
% %%

% For $\Phi=\exists y.\inadom(y)\land\Phi'$: by definition, $T_1,q_1,\vfo_1\models \Phi$
% iff, for some $d_1'$, it is the case that $T_1,q_1,\vfo_1[y/d'_1]\models \inadom(y)\land\Phi'$.
% By the induction hypothesis, the latter holds iff $T_2,q_2,\vfo_2[y/h(d'_1)]\models \inadom(y)\land\Phi'$,
% which implies $T_2,q_2,\vfo_2\models \Phi$. The other direction is proven simmetrically.

% For $\Phi=\inadom(x) \land \DIAM{\Phi'}$: assume that
% $T_1,q_1,\vfo_1\models (\inadom(x) \land \DIAM{\Phi'})$.  By
% definition, this implies that $d_1 \in \adom(\I_1(q_1))$, thus
% $\vfo_2(x)=d_2=h(d_1)$, and that there exists a transition
% $q_1 \ra_1 q'_1$ such that $T_1,q'_1,\vfo_1 \models \Phi'$.  But then,
% since $q_1 \approx q_2$, there exists a transition $q_2 \ra_2 q'_2$
% such that $q'_1 \approx q'_2$ and
% $\arestrict{\I_1}(q'_1) \sim_{h'} \arestrict{\I_2}(q'_2)$, with $h'$
% an extension of $\restrict{h}{\adom(\I_1(q_1))}$.  Since $d_1 \in \adom(\I_1(q_1))$ and
% $h'$ is an extension of $\restrict{h}{\adom(\I_1(q_1))}$, we have that
% $h'(d_1) = h(d_1)=d_2$. This implies, in turn, that
% $d_2=h'(d_1) \in \adom(\I_2(q_2))$.  
% %%
% Hence we can apply the induction
% hypothesis, using mapping $h'$, and get that $T_1,q'_1,\vfo_1 \models \Phi$ implies that $T_2,q'_2,\vfo_2\models \Phi$.  
% %%
% But then, since $q_2 \ra_2 q'_2$, we
% have that $T_2,q_2,\vfo_2 \models (\inadom(x) \land
% \DIAM{\Phi'})$. The other direction can be proven in a symmetric way.
  
% For $\Phi=\inadom(x) \land \BOX{ \Phi''}$:  
% we rewrite, for convenience, $\Phi$ as: $\lnot(\inadom(x) \limp \DIAM{ \Phi''})$, with
%   $\Phi'' = \neg \Phi'$. We then prove the thesis for the implication. 
%   Assume that $T_1,q_1,\vfo_1 \models (\inadom(x) \limp\DIAM{ \Phi'})$.
% By definition, this implies that: \myi either
% $d_1\not\in \adom(\I_1(q_1))$; 
% or \myii $d_1\in \adom(\I_1(q_1))$  and there exists a transition $q_1
%   \ra_1 q'_1$ such that $T_1,q'_1,\vfo_1 \models \Phi'$.
% We distinguish the two cases:
% \begin{itemize}
% \item If $d_1 \not\in \adom(\I_1(q_1))$ then, by lemma's hypotesis,
%   $d_2\notin\adom(\I_2(q_2))$. Hence, we have that
%   $T_2,q_2,\vfo_2 \not \models \inadom(x)$ and so
%   $T_2,q_2,\vfo_2 \models (\inadom(x) \limp \DIAM{\Phi'})$.

% \item If $d_1 \in \adom(\I_1(q_1))$, we can proceed in the 
% same way as for the case of $\Phi=\inadom(x) \land \DIAM{\Phi'}$.
% \end{itemize}
% The other direction is proven symmetrically.
% \end{proof}


\begin{lemma}\label{lemma:myhm-bisimulation}
  Consider two transition systems
  $T_1= \tup{\Delta_1,Q_1,q_{10},\ra_1,\I_1}$ and
  $T_2= \tup{\Delta_2, Q_2, q_{20}, \ra_2, \I_2}$, 
  %both with infinite object domain, 
 and two individual variable valuations $\vfo_1$ and
  $\vfo_2$ mapping variables to $\Delta_1$ and $\Delta_2$,
  respectively, and two states $q_1\in Q_1$, $q_2 \in Q_2$. If 
  $q_1 \approx q_2$ and there exists a mapping $h$ such that
  $\arestrict{\I_1}(q_1) \sim_h \arestrict{\I_2}(q_2)$, and such that
  for each individual variable $x$ we have that
  $h(\vfo_1(x))= \vfo_2(x)$, then every (open) formula
  $\Phi$ of $\myhm$ we have:
\[T_1,q_1,\vfo_1 \models \Phi \, \textrm{ if and only if }\,  T_2,q_2,\vfo_2 \models \Phi. \]
\end{lemma}
\begin{proof}
  We proceed by induction on the structure of $\Phi$. 
 
  For $\Phi=\varphi$, we observe that, by Theorem~\ref{thm:dom-ind}, 
 $\I_i(q_i),\vfo_i\models\varphi$ if and only if $\arestrict{\I_i}(q_i),\vfo_i\models\varphi'$
 ($i=1,2$),
  for $\varphi'$ the rewriting of $\varphi$ as its domain-independent version.
  Further, because $\arestrict{\I_1}(q_1)\sim_h\arestrict{\I_2}(q_2)$, 
  by the invariance of  FOL wrt isomorphic interpretations, it follows that 
  $\arestrict{\I_1}(q_1),\vfo_1\models\varphi'$ if and only if 
  $\arestrict{\I_2}(q_2),\vfo_2\models\varphi'$ (either if $d_2 = h(d_1)$ or 
  $d_i\notin \adom(\I_i(q_i))$). 
  These two facts easily imply the thesis.
%%

The cases of boolean connectives are obtained by straightforward induction keeping the same individual valuations $\vfo_1$ and $\vfo_2$ and the same mapping $h$.

For $\Phi=\exists y.\inadom(y)\land\Phi'$. Suppose that $T_1,q_1,\vfo_1\models \Phi$
then for some $d_1$, it is the case that $T_1,q_1,\vfo_1[y/d_1]\models \inadom(y)\land\Phi'$. Notice this implies that $d_1\in\adom(\I_1(q_1))$, as a result $h(d_1)=d_2$ for some $d_2\in \adom(\I_1(q_1))$. Consider the individual valuation $\vfo_2[y/d_2)]$, for every variable $x$ we have $h(\vfo_1[y/d_1](x)=\vfo_2[y/d_2)](x)$ (for $y$ we have $\vfo_2[y/d_2](y)=d_2=h(d_1)=h(\vfo_1[y/d_1](y))$). Hence using this new valuations and the same mapping $h$ we can apply the 
induction hypothesis, and conclude that $T_2,q_2,\vfo_2[y/d_2]\models \inadom(y)\land\Phi'$,
which implies $T_2,q_2,\vfo_2\models \Phi$.

On the other hand if $T_2,q_2,\vfo_2\models \Phi$ then for some $d_2'$, it is the case that $T_2,q_2,\vfo_2[y/d_2]\models \inadom(y)\land\Phi'$. Notice that $d_2\in\adom(\I_2(q_2))$ hence $h^{-1}(d_2) = d_1$ for some $d_1\in\adom(\I_1(q_1))$.  Consider the individual valuation $\vfo_1[y/d_1)]$, for every variable $x$ we have $h(\vfo_1[y/d_1](x)=\vfo_2[y/d_2)](x)$ Hence again using this new valuations and the same mapping $h$ we can apply the 
induction hypothesis, and conclude that $T_1,q_1,\vfo_1[y/d_1]\models \inadom(y)\land\Phi'$,
which implies $T_1,q_1,\vfo_1\models \Phi$.


For $\Phi=\inadom(\vec{x}) \land \DIAM{\Phi'}$. Suppose that
$T_1,q_1,\vfo_1\models (\inadom(\vec{x}) \land \DIAM{\Phi'})$.  By
definition, this implies that $\vfo_1(x_i) \in \adom(\I_1(q_1))$ for each $x_i\in\vec{x}$, thus
$\vfo_2(x_i)=h(\vfo_1(x_i))$. Moreover there exists a transition
$q_1 \ra_1 q'_1$ such that $T_1,q'_1,\vfo_1 \models \Phi'$.  But then,
since $q_1 \approx q_2$, there exists a transition $q_2 \ra_2 q'_2$
such that $q'_1 \approx q'_2$ and
$\arestrict{\I_1}(q'_1) \sim_{h'} \arestrict{\I_2}(q'_2)$, with $h'$
an extension of $\restrict{h}{\adom(\I_1(q_1))}$.  Since $\vfo_1(x_i)\in \adom(\I_1(q_1))$ and
$h'$ is an extension of $\restrict{h}{\adom(\I_1(q_1))}$, we have that
$h'(\vfo_1(x_i)) = h(\vfo_1(x_i))=\vfo_2(x_i)$. 
%%
Notice that outside $\adom(\I_1(q_1))\cup\adom(\I_1(q'_1))$, the
mapping $h'$ is arbitrary, so we can choose it such that for all
variables $x$ we have $(h'(\vfo_1(x)=h(\vfo_2(x))$.  With this new
mapping $h'$ we can apply the induction hypothesis, and get that
$T_1,q'_1,\vfo_1 \models \Phi$ implies that
$T_2,q'_2,\vfo_2\models \Phi$, and since $q_2 \ra_2 q'_2$, we have
that $T_2,q_2,\vfo_2 \models (\inadom(x) \land \DIAM{\Phi'})$.  

Suppose that
$T_2,q_2,\vfo_2\models (\inadom(\vec{x}) \land \DIAM{\Phi'})$. This implies that $\vfo_2(x_i) \in \adom(\I_2(q_2))$ for each $x_i\in\vec{x}$, thus
$h^{-1}\vfo_2(x_i)=\vfo_1(x_i)\in \adom(\I_1(q_1))$. Moreover there exists a transition
$q_2 \ra_2 q'_2$ such that $T_2,q'_2,\vfo_2 \models \Phi'$.  But then,
since $q_1 \approx q_2$, there exists a transition $q_1 \ra_1 q'_1$
such that $q'_1 \approx q'_2$ and
$\arestrict{\I_1}(q'_1) \sim_{h'} \arestrict{\I_2}(q'_2)$, with $h'$
an extension of $\restrict{h}{\adom(\I_1(q_1))}$.  Since $\vfo_1(x_i)\in \adom(\I_1(q_1))$ and
$h'$ is an extension of $\restrict{h}{\adom(\I_1(q_1))}$, we have that
$h'(\vfo_1(x_i)) = h(\vfo_1(x_i))=\vfo_2(x_i)$. 
%%
Again outside $\adom(\I_1(q_1))\cup\adom(\I_1(q'_1))$, the
mapping $h'$ is arbitrary, so we can choose it such that for all
variables $x$ we have $(h'(\vfo_1(x)=h(\vfo_2(x))$.  With this new
mapping $h'$ we can apply the induction hypothesis, and get that
$T_1,q'_1,\vfo_1 \models \Phi$ implies that
$T_2,q'_2,\vfo_2\models \Phi$, and since $q_2 \ra_2 q'_2$, we have
that $T_2,q_2,\vfo_2 \models (\inadom(x) \land \DIAM{\Phi'})$.  
%%
% The other direction can be proven in a symmetric way, again using the
% fact that $h$ and $h'$ are invertible over $\adom(\I_1(q_1))$ and
% $\adom(\I_1(q_1))\cup\adom(\I_1(q'_1))}$, respectively.
  
For $\Phi=\inadom(\vec{x}) \land \BOX{ \Phi''}$:  
we rewrite, for convenience, $\Phi$ as: $\lnot(\inadom(\vec{x}) \limp \DIAM{ \Phi''})$, with
  $\Phi'' = \neg \Phi'$. We then prove the thesis for the implication. 
  Assume that $T_1,q_1,\vfo_1 \models (\inadom(\vec{x}) \limp\DIAM{ \Phi'})$.
By definition, this implies that: \myi either for some  $x_i\in\vec{x}$ we have
$\vfo_1(x_i)\not\in \adom(\I_1(q_1))$; 
or \myii for all $x_i\in\vec{x}$ we have $\vfo_1(x_i)\in \adom(\I_1(q_1))$  and there exists a transition $q_1 \ra_1 q'_1$ such that $T_1,q'_1,\vfo_1 \models \Phi'$.
We distinguish the two cases:
\begin{itemize}
\item If for some $x_i\in\vec{x}$,
  $\vfo_1(x_i)\not\in \adom(\I_1(q_1))$, then we have also that $\vfo_2(x_i)\not\in \adom(\I_2(q_2))$. Indeed, assume toward contradiction that $\vfo_2(x_i) \in\adom(\I_2(q_2))$.  Since $\arestrict{\I_1}(q_1) \sim_h \arestrict{\I_2}(q_2)$ it follows that inverse $h^{-1} $ of $h$ is unique $\vfo_2(x_i)$ hence  $h^{-1}(\vfo_2(x_i))=\vfo_1(x_i)$ and $\vfo_1(x_i) \in \adom(\I_1(q_1))$, getting a contradiction.
So we have that
  $T_2,q_2,\vfo_2 \not \models \inadom(\vec{x})$ and so
  $T_2,q_2,\vfo_2 \models (\inadom(\vec{x}) \limp \DIAM{\Phi'})$.

\item If for all $x_i\in\vec{x}$, $\vfo_i(x_i)\in \adom(\I_1(q_1))$, we can proceed in the 
same way as for the case of $\Phi=\inadom(\vec{x}) \land \DIAM{\Phi'}$.
\end{itemize}
The other direction is proven symmetrically.
\end{proof}

We can now extend the result to the whole $\mymu$.
%%
\begin{lemma}\label{lemma:mymu-bisimulation}
  Consider two transition systems
  $T_1= \tup{\Delta_1,Q_1,q_{10},\ra_1,\I_1}$ and
  $T_2= \tup{\Delta_2, Q_2, q_{20}, \ra_2, \I_2}$, 
  %both with infinite object domain, 
 and two individual variable valuations $\vfo_1$ and
  $\vfo_2$ mapping variables to $\Delta_1$ and $\Delta_2$,
  respectively, and two states $q_1\in Q_1$, $q_2 \in Q_2$. If 
  $q_1 \approx q_2$ and there exists a mapping $h$ such that
  $\arestrict{\I_1}(q_1) \sim_h \arestrict{\I_2}(q_2)$, and such that
  for each individual variable $x$ we have that
  $h(\vfo_1(x))= \vfo_2(x)$, then every (open) formula
  $\Phi$ of $\mymu$ we have:
\[T_1,q_1,\vfo_1 \models \Phi \, \textrm{ if and only if }\,  T_2,q_2,\vfo_2 \models \Phi. \]
\end{lemma}
\begin{proof}
  We prove the theorem in two steps. First, we show that Lemma
  \ref{lemma1:myhm-bisimulation} can be extended to the infinitary
  version of $\myhm$ that supports arbitrary 
  disjunction. Then, we recall that fixpoints can be translated into
  this infinitary logic, thus guaranteeing invariance for the whole
  $\mymu$ logic.
%%
  Let $\Psi$ be a  set of  $\mymu$ formulas sharing the same  open individual variables. Given a
  transition system $T =
  \tup{\Delta,Q,q_0,\ra,\I}$, the semantics of
  $\bigvee \Psi$ is $\MODAT{\bigvee \Psi} = \bigcup_{\psi \in
    \Psi} \MODAT{\psi}$. Therefore, given a state $q$ of $T$
  and a variable valuation $\vfo$ that assigns to each free variable
  of $\Psi$ a value $d \in \adom(\I(q))$ , we have $T,q,\vfo \models
  \Psi$ if and only if $T,q,\vfo \models \psi$ for some $\psi
  \in \Psi$. Arbitrary  conjunction is obtained for free
  through negation.
%%
  Lemma~\ref{lemma1:myhm-bisimulation} extends to this arbitrary
   disjunction.  By induction hypothesis, under the
  assumption of the Lemma, we can assume that for every formula
  $\psi \in \Psi$, we have $T_1,q_{10},\vfo_1 \models \psi$ if and
  only if $T_2,q_{20},\vfo_2 \models \psi$.  Given the semantics of
  $\bigvee \Psi$ above, this implies that
  $T_1,q_{10},\vfo_1 \models \bigvee \Psi$ if and only if
  $T_2,q_{20},\vfo_2 \models \bigvee \Psi$.

  In order to extend the result to the whole $\mymu$, we resort to the
  well-known result stating that fixpoints of the $\mu$-calculus can
  be translated into the infinitary Hennessy-Milner Logic by iterating
  over \emph{approximants} (see~\cite{BS07}), where the approximant
  of index $\alpha$ is denoted by $\mu^\alpha Z.\Phi$ for least
  fixpoint formulas $\mu Z.\Phi$ and $\nu^\alpha Z.\Phi$ for greatest
  fixpoint formulas $\nu Z.\Phi$. This is a standard result that holds
  also for $\mymu$. In particular, approximants are built as follows:
\[\begin{array}{rcl@{\qquad}rcl}
  \mu^0 Z.\Phi & = & \false 
  &  \nu^0 Z.\Phi & =& \true\\
  \mu^{\beta+1} Z.\Phi & =& \Phi[Z/\mu^\beta Z.\Phi]
  & \nu^{\beta+1} Z.\Phi & =& \Phi[Z/\nu^\beta Z.\Phi]\\
  \mu^\lambda Z.\Phi & =& \bigvee_{\beta < \lambda} \mu^\beta Z. \Phi 
  &
  \nu^\lambda Z.\Phi & =& \bigwedge_{\beta < \lambda} \nu^\beta Z. \Phi
\end{array}
\]
where $\lambda$ is a limit ordinal, and the notation $\Phi[Z/\nu^\beta Z.\Phi]$ denotes the formula obtained from $\Phi$ by replacing each occurrence of $Z$ by $\nu^\beta Z.\Phi$.
%%
By Tarski\&Knaster Theorem~\cite{Tarski55}, the fixpoints and their
approximants are connected by the following properties: given a
transition system $T$ and a state $q$ of $T$,
\begin{itemize}
\item $q \in \MODAT{\mu Z.\Phi}$ if and only if there exists an
  ordinal $\alpha$ such that $s \in \MODAT{\mu^\alpha Z.\Phi}$ and, for
  every $\beta < \alpha$,  it holds that $s \not\in \MODA{\mu^\beta Z.\Phi}$;
\item $q \not\in \MODAT{\nu Z.\Phi}$ if and only if there exists an ordinal $\alpha$ such that $s \not\in \MODAT{\nu^\alpha
    Z.\Phi}$ and, for every $\beta < \alpha$, it holds that $q \in \MODA{\nu^\beta
    Z.\Phi}$.
\end{itemize}
%Then we get the result, along the line of reasoning of Lemma~\ref{lemma1:myhm-bisimulation}.
\end{proof}

With this lemma in place we can prove the invariance results. 


\begin{theorem}
\label{thm:mymu-bisimulation}
Consider two transition systems $T_1=\tup{\Delta_1,Q_1,q_{10},\ra_1,\I_1}$ 
and $T_2=\tup{\Delta_2,Q_2,q_{20},\ra_2,\I_2}$.
If $T_1 \approx T_2$,
then, for every $\mymu$ closed formula $\Phi$,
$T_1 \models \Phi \textrm{ if and only if } T_2 \models \Phi.$
\end{theorem}
\begin{proof}
  By Lemma~\ref{lemma:mymu-bisimulation}: if $T_1 \approx T_2$ then
  $q_{10} \approx q_{20}$. This implies that there exists a mapping
  $h$ such that
  $\arestrict{\I_1}(q_{10})\sim_h\arestrict{\I_2}(q_{20})$.  Now
  consider individual valuations $\vfo_1$ and $\vfo_2$ on $\Delta_1$
  and $\Delta_2$, respectively. (Notice that since we are
  considering closed formulas $\Phi$ such individual valuations are
  irrelevant in evaluating $\Phi$.)  In particular lets define them as follows  for all $x$ the individual valuation $\vfo_1(x)=d_1$ for some $d_1\notin \adom(\I_1(q_{10}))$, analogously, for all $x$ the valuation  $\vfo_2(x)=d_2$ for some $d_2\notin \adom(\I_2(q_{20}))$.
  Without loss of generality we may assume that $h(d_1)=d_2$.
Hence we can apply Lemma~\ref{lemma:mymu-bisimulation}, thus getting the thesis.
\end{proof}

Thus, to check whether a transition system $T$ satisfies a $\mymu$ formula $\Phi$,
one can perform the check on any transition system $T'$ that is bisimilar to $T$. This is 
particularly useful in those cases where $T$ is infinite-state but admits some 
finite-state bisimilar transition system. We exploit this result later on.



%%% Local Variables:
%%% mode: latex
%%% dirvars: nil
%%% save-place: t
%%% TeX-master: "main"
%%% End:


